Signature Cocycles on the Mapping Class Group and Symplectic Groups

Werner Meyer constructed a cocycle in $H^2(Sp(2g, \mathbb{Z}); \mathbb{Z})$ which computes the signature of a closed oriented surface bundle over a surface, with fibre a surface of genus g. By studying properties of this cocycle, he also showed that the signature of such a surface bundle is a multiple of 4. In this paper, we study the signature cocycles both from the geometric and algebraic points of view. We present geometric constructions which are relevant to the signature cocycle and provide an alternative to Meyer's decomposition of a surface bundle. Furthermore, we discuss the precise relation between the Meyer and Wall-Maslov index. The main theorem of the paper, Theorem 6.6, provides the necessary group cohomology results to analyze the signature of a surface bundle modulo any integer N. Using these results, we are able to give a complete answer for N = 2, 4 and 8, and based on a theorem of Deligne, we show that this is the best we can hope for using this method.

==> paper3-6.tex <==
%PAPER3-6.TEX (3.9.2018)
%OWNER Caterina

\section{The signature of a surface bundle modulo eight}\label{se:recipe}


Let $\Sigma_g \to E \to \Sigma_h$ be a surface bundle, with fibre
the surface $\Sigma_g$  of genus $g \geqslant 1$, and base the surface $\Sigma_h$ of genus $h \geqslant 1$.
We shall use the $\bZ/4$-coefficient monodromy
$$\pi_1(\Sigma_h) \longrightarrow \mcg{g} \longrightarrow \Sp(2g,\bZ) \longrightarrow \Sp(2g,\bZ/4)$$
to provide a recipe for computing the signature
of the $4$-manifold $E$ modulo eight.


We start with some generalities about central group extensions and commutators.



For any abelian group $A$ there is defined a cap product pairing
$$H^2(\Sigma_h;A)\times H_2(\Sigma_h) \longrightarrow H_0(\Sigma_h;A)=A~;\left(\sigma,\left[\Sigma_h\right]\right) \longmapsto
\left\langle \sigma,\left[\Sigma_h\right]\right\rangle$$
with $[\Sigma_h] \in H_2(\Sigma_h)$ the fundamental class. In the first instance, we obtain a formula for
$\left\langle \sigma,\left[\Sigma_h\right]\right\rangle \in A$ in terms of the central extension
$$1 \longrightarrow A \longrightarrow \pi_1(\Sigma_h)_\sigma \longrightarrow \pi_1(\Sigma_h) \longrightarrow 1$$
classified by $\sigma \in H^2(\Sigma_h;A)=H^2(\pi_1(\Sigma_h);A)$. 
The fundamental group of $\Sigma_h$  is the one relator
group\index{one relator group} given by
\[ \pi_1(\Sigma_h)=\left\langle a_1,b_1,a_2,b_2,\dots,a_h,b_h\mid r\right\rangle \]
where $r= [a_1,b_1][a_2,b_2]\cdots[a_h,b_h]$ is the single relator.

\begin{lemma}\label{le:fundamental} 
{\rm (i)} The central extension classified by $1 \in H^2(\pi_1(\Sigma_h);\bZ)\cong \bZ$ 
$$1 \longrightarrow \bZ \stackrel{i}{\longrightarrow} \pi_1(\Sigma_h)_1 \stackrel{p}{\longrightarrow} \pi_1(\Sigma_h) \longrightarrow 1$$
is given by
$$\begin{array}{l}
\pi_1(\Sigma_h)_1=\left\langle a_1,b_1,\dots,a_h,b_h,r\,\vert\, [a_1,r],\dots,[b_h,r],r=[a_1,b_1]\cdots[a_h,b_h]\right\rangle,\\[1ex]
i\colon \bZ \longrightarrow \pi_1(\Sigma_h)_1~;~1 \longmapsto r~.
\end{array}$$
{\rm (ii)} Let $1 \to A \to \pi_1(\Sigma_h)_\sigma \to \pi_1(\Sigma_h) \to 1$ be the central extension
classified by an element
$$\sigma \in H^2(\Sigma_h;A)\cong H^2(\pi_1(\Sigma_h);A)\cong\mathsf{Hom}(H_2(\pi_1(\Sigma_h)), A)\cong A~.$$
Then
$$\pi_1(\Sigma_h)_{\sigma}=\mathsf{coker}\left(\bZ \longrightarrow  \pi_1(\Sigma_h)_1 \times A\right)$$
fits into a morphism of central extensions
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r]^-i\ar[d]^-{\sigma} & 
\pi_1(\Sigma_h)_1 \ar[r]^-p \ar[d]^-{\chi} & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1 \\
1 \ar[r] & A \ar[r]^-{i_\sigma} & \pi_1(\Sigma_h)_\sigma \ar[r]^-{p_\sigma} & \pi_1(\Sigma_h) \ar[r] & 1} \]
such that
$$\left\langle \sigma,\left[\Sigma_h\right] \right\rangle=\chi\left([a_1,b_1][a_2,b_2] \cdots [a_h,b_h]\right) \in A \subset \pi_1(\Sigma_h)_\sigma~.$$
{\rm (iii)} For any group $\bar{G}$, abelian group $A$ and cohomology class $c \in H^2(\bar{G};A)$ let
$$1 \longrightarrow A \longrightarrow G \stackrel{p}{\longrightarrow} \bar{G} \longrightarrow 1$$
be the central extension of $\bar{G}$ by $A$ classified by $c$. 
A group morphism $\bar{f}\colon\pi_1(\Sigma_h) \to \bar{G}$ is determined
by elements $u_1,v_1,\dots,u_h,v_h \in  G$ such that
$[u_1,v_1]\cdots [u_h,v_h] \in A$, with $\bar{f}(a_i)=p(u_i)$, $\bar{f}(b_i)=p(v_i)$. The pullback central extension $H$ of $\pi_1(\Sigma_h)$ by $A$
\[ \xymatrix@R=6mm{1 \ar[r] & A \ar[r] \ar@{=}[d] & H \ar[r] \ar[d]^-{f} & \pi_1(\Sigma_h) \ar[r] \ar[d]^-{\bar{f}} & 1 \\
1 \ar[r] & A \ar[r]^{i_c} &  G\ar[r]^{p_c}  & \bar{G} \ar[r] & 1} \]
is classified by
$$\bar{f}^*(c)= [u_1,v_1]\cdots[u_h,v_h] \in H^2(\pi_1(\Sigma_h);A)\cong A$$
so that $H=\pi_1(\Sigma_h)_{\bar{f}^*(c)}$.
\end{lemma}
\begin{proof} (i) This can be seen by construction. We propose also a more general method that will be useful in the rest of the proof.

Since $h\geqslant 1$, $\Sigma_h$ is
a $K(\pi_1(\Sigma_h),1)$, so that
$$H_1(\pi_1(\Sigma_h))=H_1(\Sigma_h)=\bZ^{2h}~,~H_2(\pi_1(\Sigma_h))=H_2(\Sigma_h)=\bZ~.$$
In particular,
\[ \Ext^1_{\bZ}(H_1(\pi_1(\Sigma_h)),H_2(\pi_1(\Sigma_h)))=0, \]
and so the universal coefficient sequence shows that
\[ H^2(\pi_1(\Sigma_h); H_2(\pi_1(\Sigma_h))) \longrightarrow \Hom_\bZ(H_2(\pi_1(\Sigma_h)),H_2(\pi_1(\Sigma_h))) \]
is an isomorphism. In particular, lifting the identity homomorphism gives
a well defined generator of $H^2(\pi_1(\Sigma_h);\bZ)\cong \bZ$,
corresponding to the  central extension  $1 \to \bZ \to \pi_1(\Sigma_h)_1 \to \pi_1(\Sigma_h) \to 1$ of the statement.

Recall that if $G$ is a quotient of a free group $F$ by relations $R$ then $H_2(G)=R\cap[F,F]/[R, F]$. If $R\subseteq [F,F]$ there is a canonical central
extension
$$1 \longrightarrow H_2(G)=R/[R,F] \longrightarrow  \widetilde{G}=F/[R,F] \longrightarrow  G=F/R \longrightarrow  1$$
classified by $1 \in H^2(G;H_2(G)) \cong  \Hom_\bZ(H_2(G),H_2(G))$.
In particular, for $G=\pi_1(\Sigma_h)$, $H_2(G)=\bZ$, this gives the extension $\pi_1(\Sigma_h)_1$
with the presentation in the statement of (i).\\
\indent 
(ii) We are considering the cokernel of the natural map $$\bZ\ni n\longmapsto \left(r^n, \sigma(n)\right)\in \pi_1(\Sigma_h)_1 \times A.$$ The map $i_\sigma$ is given by $a\mapsto [(1, -a)]$, the map $p_\sigma$ by $[(u, a)]\mapsto p(u)$ and $\chi$ by $u\mapsto [(u, 0)]$.

Let $s\colon\pi_1(\Sigma_h)\rightarrow \pi_1(\Sigma_h)_1$ be a section of $p$, with associated cocycle $m\colon \pi_1(\Sigma_h)\times \pi_1(\Sigma_h)\rightarrow \bZ$ satisfying $i(m(x, y))=s(x)s(y)s(xy)^{-1}$. The composition $\chi\circ s$ is a section of $p_\sigma$.
We compute the associated cocycle:
$$\chi s(x)\chi s(y)\chi s(xy)^{-1}=\chi\left(s(x)s(y)s(xy)^{-1}\right)=\chi\left(i(m(x, y))\right)=i_\sigma\left(\sigma(m(x, y))\right).$$

This shows that the group extension $\mathsf{coker}\left(\bZ \rightarrow  \pi_1(\Sigma_h)_1 \times A\right)$ corresponds to $\sigma$.

%Now given an abelian group $A$ and an element $\sigma\in H^2(\pi_1(\Sigma_h); A)$, 
We can evaluate
$\sigma$ on $[\Sigma_h]\in H_2(\pi_1(\Sigma_h))$ via the induced map in $\mathsf{Hom}(H_2(\pi_1(\Sigma_h)), A)$: we have obtained a lifting $\chi$ of $p$
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r]^-i \ar[d]^\sigma & \pi_1(\Sigma_h)_1 \ar[r]^p \ar[d]^\chi & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1 \\
1 \ar[r] & A \ar[r]^-{i_\sigma} & \pi_1(\Sigma_h)_{\sigma} \ar[r]^{p_\sigma} & \pi_1(\Sigma_h) \ar[r] & 1} \]
with $\bZ \to A;1 \mapsto \left\langle \sigma,\left[\Sigma_h\right]\right\rangle=i_\sigma^{-1}\left(\chi\left([a_1,b_1][a_2,b_2] \cdots [a_h,b_h]\right)\right)$.\\

{\rm (iii)} Apply (ii) with $\sigma=\bar{f}^*(c) \in H^2(\pi_1(\Sigma_h);A)$: consider the commutative diagram
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r] \ar[d]^\sigma & \pi_1(\Sigma_h)_1 \ar[r] \ar[d]^-{\chi} & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1\phantom{.} \\
1 \ar[r] & A \ar[r] \ar@{=}[d] & \pi_1(\Sigma_h)_\sigma \ar[r] \ar[d]^-{f} & \pi_1(\Sigma_h) \ar[r] \ar[d]^-{\bar{f}} & 1\phantom{.} \\
1 \ar[r] & A \ar[r]^{i_c} & G\ar[r]^{p_c}  & \bar{G} \ar[r] & 1.} \]
The morphism $f$ is given by $[(a_i, 0)], [(b_i, 0)], [(1, -a)]\mapsto u_i, v_i, i_c(a)$ respectively. Note then that
\begin{align*}
\left\langle \bar{f}^*(c),\left[\Sigma_h\right] \right\rangle
&=\left\langle\sigma,\left[\Sigma_h\right] \right\rangle\\
&= i_\sigma^{-1}\left(\chi\left([a_1,b_1][a_2,b_2]\cdots[a_h,b_h]\right)\right) 
\end{align*}
which is mapped to $G$ via $i_c$ to
$[u_1,v_1]\cdots[u_h,v_h] \in i_c(A)\cong A\cong H^2(\pi_1(\Sigma_h);A)$.
\end{proof}

Let $N \geqslant 0$; for $N=0$, $\bZ/N$ is the infinite cyclic group, and for $N \geqslant 1$, $\bZ/N$ is the finite cyclic group of order $N$. 

\begin{eg}\label{le:extensionbyzN}
The central extension
$$1 \longrightarrow \bZ/N \longrightarrow \widetilde{\pi_1(\Sigma_h)} \longrightarrow \pi_1(\Sigma_h) \longrightarrow 1$$
classified by $1 \in H^2(\pi_1(\Sigma_h);\bZ/N)=\bZ/N$ is
$$\begin{array}{l}
\widetilde{\pi_1(\Sigma_h)}=\left\langle a_1,b_1,\dots,a_h,b_h,r\,\vert\, [a_1,r],\dots,[b_h,r],r=[a_1,b_1]\cdots[a_h,b_h],r^N\right\rangle,\\[1ex]
\bZ/N \longrightarrow \widetilde{\pi_1(\Sigma_h)}~;~1 \longmapsto r~.
\end{array}$$
\end{eg}

Meyer \cite{Meyer:1973a} proved that $\sigma(E)=0$ for a surface bundle $\Sigma_g \to E \to \Sigma_h$ with $g \leqslant 2$. 

\begin{lemma} \label{le:symplectic}
Let $g \geqslant 3$.\\
{\rm (i)} The cohomology class
$$[\tau_g]=4 \in H^2(\Sp(2g,\bZ);\bZ) \cong  \bZ$$
 corresponds to the central extension
\[ 1 \longrightarrow \bZ \longrightarrow \Sp(2g,\bZ)_4 \longrightarrow \Sp(2g,\bZ) \longrightarrow 1\]
with cocycle determined by the signatures of the double mapping tori
$$\tau_g\colon\Sp(2g,\bZ) \times \Sp(2g,\bZ) \longrightarrow \bZ~;~(\alpha,\beta) \longmapsto
-\sigma(T(\alpha,\beta))~.$$
{\rm (ii)} For a surface bundle $F=\Sigma_g \to E \to B=\Sigma_h$
$$\sigma(E)=-\left\langle \bar\chi^*\left([\tau_g]\right),\left[\Sigma_h\right] \right\rangle \in 4\bZ$$
with $\bar\chi\colon\pi_1(\Sigma_h) \to \Sp(2g,\bZ)$ the monodromy. The cohomology class
$\bar\chi^*([\tau_g]) \in H^2(\pi_1(\Sigma_h);\bZ)$ classifies the extension
$$1 \longrightarrow \bZ \longrightarrow \pi_1(\Sigma_h)_{\bar\chi(4)} \longrightarrow \pi_1(\Sigma_h) \longrightarrow 1$$
with cocycle
$$\pi_1(\Sigma_h) \times \pi_1(\Sigma_h) \longrightarrow \bZ ~;~
(\alpha,\beta) \longmapsto -\sigma\left(T\left(\bar\chi(\alpha),\bar\chi(\beta)\right)\right).$$
For $\bar \chi(a_i)=u_i$, $\bar \chi(b_i)=v_i \in  \Sp(2g,\bZ)$
this is the pullback of the central extension of $\Sp(2g,\bZ)$ in {\rm (i)}
$$\xymatrix{
1 \ar[r] & \bZ \ar@{=}[d] \ar[r] & \pi_1(\Sigma_h)_{\bar\chi(4)} \ar[r] \ar[d] & \pi_1(\Sigma_h) \ar[d]^{\bar\chi} \ar[r] & 1 \\
1 \ar[r] & \bZ \ar[r] & \Sp(2g,\bZ)_4 \ar[r]^-{p} & \Sp(2g,\bZ)\ar[r] & 1}$$
with
$$\left(-\sigma(E),1\right)=
\left(0,u_1\right)\left(0, v_1\right)\left(0, u_1^{-1}\right)\left(0, v_1^{-1}\right)\cdots\left(0,u_h\right)\left(0, v_h\right)\left(0, u_h^{-1}\right)\left(0,v_h^{-1}\right) \in
\Sp(2g,\bZ)_4~.$$
{\rm (iii)} The $\bZ/2$-reduction  of $[\tau_g]/4$
$$[\tau_g]/4=\begin{cases}
(1,0)\\
1 \\
\end{cases} \in
H^2(\Sp(2g,\bZ);\bZ/2) \cong \begin{cases} 
\bZ/2 \oplus \bZ/2  &\mbox{if }g=3, \\
  \bZ/2 &\mbox{if }  g\geqslant 4\phantom{,} \end{cases}$$
 corresponds to the  central extension
\[ 1 \longrightarrow \bZ/2 \longrightarrow \widetilde{\widetilde{\Sp(2g,\bZ)}} \longrightarrow \Sp(2g,\bZ) \longrightarrow 1\]
such that for a surface bundle $\Sigma_g \to M \to \Sigma_h$
$$\sigma(E)/4=\left\langle \bar \chi^*\left([\tau_g]/4\right),\left[\Sigma_h\right] \right\rangle \in \bZ/2~.$$
\end{lemma}
\begin{proof} (i)+(ii) Meyer \cite{Meyer:1973a}.\\
(iii) From (i) we have that $[\tau_g]/4=1\in H^2(\Sp(2g,\bZ); \bZ)\cong\bZ$ is the generator of this cohomology group. By naturality of the universal coefficient theorem and because the group $\Sp(2g,\bZ)$ is perfect for $g\geq3$, one has a commutative diagram
$$
\xymatrix
{
H^2(\Sp(2g,\bZ); \bZ)\ar[r]^{r_2}\ar[d]^\cong &H^2(\Sp(2g,\bZ); \bZ/2)\ar[d]^\cong\\
\mathsf{Hom}(H_2(\Sp(2g, \bZ); \bZ), \bZ)\ar[r]^{r_2}& \mathsf{Hom}(H_2(\Sp(2g, \bZ); \bZ), \bZ/2).
}
$$
Lemma \ref{Lemma:co-homology computations}\eqref{H_2 Sp Z Z}, \eqref{H^2 Sp Z Z} and \eqref{H^2 Sp Z Z/2} gives
$$H_2(\Sp(2g, \bZ); \bZ)=\begin{cases}
													\bZ\oplus\bZ/2 & \mbox{if }  g=3,\\
													\bZ & \mbox{if }  g\geq 4,
															\end{cases}$$
$H^2(\Sp(2g, \bZ); \bZ)=\bZ$ if $g\geq3$,
and 
$$H^2(\Sp(2g, \bZ); \bZ/2)=\begin{cases}
													\bZ/2\oplus\bZ/2 & \mbox{if } g=3,\\
													\bZ/2 & \mbox{if }  g\geq 4.
															\end{cases}$$
Consulting Lemma \ref{Lemma:co-homology computations}\eqref{H^2 Sp image r2}, the map $r_2$ has image $$\begin{cases}
													\bZ/2\oplus\{0\} & \mbox{if } g=3,\\
													\bZ/2 & \mbox{if } g\geq 4\phantom{,}
															\end{cases}$$
and $r_2([\tau_g]/4)$ is \begin{equation*}\begin{cases}
													(1, 0) & \mbox{if } g=3,\\
													1 & \mbox{if } g\geq 4.
														\end{cases} \qedhere \end{equation*}
\end{proof}




==> paper3-7.tex <==
%PAPER3-7.TEX (8.11.2018)
%OWNER

\section{Signature of surface bundles modulo an integer}\label{se:proofs}

\subsection{Signatures of surface bundles mod $N$ for $N\leq 8$}\label{N<=8}
In \cite{BensonCampagnoloRanickiRovi:2017a} we showed the existence of a cohomology class in the second cohomology group of a finite quotient $\fH$ of $\Sp(2g, \bZ)$ that computes the mod 2 reduction of signature/4 for a surface bundle over a surface.

We recall this theorem in detail hereafter. It chases the cohomology class from the finite group
$\fH=\Sp(2g,\bZ)/\fK$ to Meyer's class on $\Sp(2g,\bZ)$.
We include details of low genus cases, which makes the theorem a
little hard to follow, so afterwards we summarise the situation
in a diagram valid for
$g\geqslant 4$.
% Based on this theorem, the recipe for computing the
%signature of $M$ modulo eight is given in Section \ref{se:recipe}.

As in \cite{BensonCampagnoloRanickiRovi:2017a} we write $\Gamma(2g,N)\unlhd\Sp(2g,\bZ)$ for the \emph{principal congruence subgroup}
consisting of symplectic matrices which are congruent to the identity
modulo $N$.
\begin{defn} \label{def:fK and fY}
For $g\geqslant 1$ we write $\fK$ (resp. $\fY$) for the subgroup of $\Sp(2g,\bZ)$ (resp. $\Sp(2g,\bZ/4)$) consisting of
matrices
\[ \begin{pmatrix} I+2\mra & 2\mrb \\ 2\mrc & I+2\mrd \end{pmatrix} \in
  \Sp(2g,\bZ)\, {\rm (}\mbox{resp. } \Sp(2g,\bZ/4){\rm )} \]
satisfying:
\begin{enumerate}
\item[\rm (i)] The vectors of diagonal entries $\Diag(\mrb)$ and $\Diag(\mrc)$ are even, and
\item[\rm (ii)] the trace $\Tr(a)$ is even (equivalently, $\Tr(d)$ is even).
\end{enumerate}
\end{defn}

\begin{theorem}\label{th:main}\ 

\begin{enumerate}
\item[\rm (i)] $\fK$  (resp. $\fY$) is a normal subgroup of $\Sp(2g,\bZ)$ (resp. $\Sp(2g,\bZ/4)$). We write
$\fH$ for the quotient $\Sp(2g,\bZ)/\fK\cong\Sp(2g,\bZ/4)/\fY$.
\item[\rm (ii)] The quotient $\Gamma(2g,2)/\fK \leq \fH$ is an elementary abelian
  $2$-group $(\bZ/2)^{2g+1}$.
\item[\rm (iii)] There are commutative braids of extensions
\index{sp2gZ2@$\fsp(2g,\bbZ{2})$}
\medskip

\[  \braid{\Gamma(2g,4)}{\Sp(2g,\bZ)}{\fH}{\fK}{\Sp(2g,\bbZ{4})}{\fY}\qquad
  \braid{\fY}{\Sp(2g,\bbZ{4})}{\Sp(2g,\bbZ{2})}{\fsp(2g,\bbZ{2})}{\fH}{(\bbZ{2})^{2g+1}}\]

\item[\rm (iv)] The extension
\[ 1 \longrightarrow (\bZ/2)^{2g+1} \longrightarrow\fH \longrightarrow \Sp(2g,\bbZ{2}) \longrightarrow 1 \]
does not split. The finite groups in the braids have orders
\[ \begin{array}{l}
\vert \Sp(2g,\bbZ{2}) \vert=2^{g^2}\prod\limits^g_{i=1}(2^{2i}-1)~,~\vert \Sp(2g,\bbZ{4}) \vert=2^{g(3g+1)}\prod\limits^g_{i=1}(2^{2i}-1)~,\\
\vert \fH \vert=2^{(g+1)^2}\prod\limits^g_{i=1}(2^{2i}-1)~,~
\vert \fY\vert =2^{(2g+1)(g-1)}~,~\vert \fsp(2g,\bbZ{2}) \vert = 2^{g(2g+1)}~.
\end{array} \]
In particular, for $g=1$
\[ \vert \Sp(2,\bbZ{2}) \vert=6,~\vert \Sp(2,\bbZ{4}) \vert=\vert
\fH \vert=48, ~\vert \fY \vert =1,~\vert\fsp(2,\bbZ{2})\vert=8. \]
\item[\rm (v)] The group $\fH$ has a double cover\index{H@$\tilde\fH$, double cover of $\fH$}
\[ 1 \longrightarrow \bbZ{2} \longrightarrow \tilde\fH \longrightarrow \fH \longrightarrow 1 \]
which is a non-split extension of $\Sp(2g,\bbZ{2})$ by an almost
extraspecial group 
$E$\index{E@$E$, almost extraspecial group}\index{almost extraspecial group} 
of order $2^{2g+2}$; namely $E$
is a central product of $\bbZ{4}$ with an
extraspecial group\index{extraspecial group} of order $2^{2g+1}$.
Furthermore, the conjugation action of $\tilde\fH$
on $E$ induces an isomorphism between $\tilde\fH/Z(\tilde\fH) \cong \fH/Z(\fH)$
and the index two subgroup of
$\Aut(E)$ centralising $Z(\tilde\fH)=Z(E)$. The groups fit into a
commutative braid of extensions\medskip
\[ \braid{\bbZ{2}}{\tilde\fH}{\Sp(2g,\bbZ{2})}{E}{\fH}{(\bbZ{2})^{2g+1}} \]
\item[\rm (vi)] For $g\geq 1$, the cohomology class in $H^2(\fH;\bbZ{2})$ determined by
the central extension $\tilde\fH$ inflates to a non-zero class 
$[\tau_g^4] \in H^2(\Sp(2g,\bbZ{4});\bbZ{2})$,\index{tau@$\tau_4 \in H^2(\Sp(2g,\bbZ{4});\bbZ{2})$} 
to a non-zero class in 
$H^2(\Sp(2g,\bZ);\bbZ{2})$, and also to a non-zero class in $H^2(\mcg{g};\bbZ{2})$ for $g\neq 2$.
If $\fX$\index{X@$\fX$, double cover of $\Sp(2g,\bbZ{4})$} 
denotes the double cover of $\Sp(2g,\bbZ{4})$ corresponding to $[\tau_g^4]$, we have:
\[ \braidtwo{\bbZ{2}}{\tilde\fH}{\mathfrak{X}}{\fH}{\fY}{\Sp(2g,\bbZ{4})} \]

\bigskip

\item[\rm (vii)]\todo[inline]{Isomorphism for g=1? Values for big n and g=1? Mail of Dave, 7.9.18}For $n\geq 2$, the inflation map induces an isomorphism
\[ H^2(\fH;\bbZ{2}) \cong H^2(\Sp(2g,\bbZ{2^n});\bbZ{2})
\cong \begin{cases} \bbZ{2} \oplus \bbZ{2} & \mbox{if } g=1, \\ \bbZ{2} \oplus \bbZ{2}
  \oplus \bbZ{2} & \mbox{if }g=2, \\ \bbZ{2} \oplus \bbZ{2} & \mbox{if }g=3, \\
\bbZ{2} & \mbox{if }g\geqslant 4.\end{cases} \]
%The extra copies of $\bZ/2$ in low genus are inflations from the
%cohomology of the quotient $\Sp(2g,\bZ/2)$
%(cf.\ Lemma \ref{le:H^2Sp2gF2}).
\item[\rm (viii)]  For $g \geqslant 3$ the inclusion of $\bZ/2$ in $\bZ/8$ sending $1$ to $4$ induces an isomorphism
\[ H^2(\Sp(2g,\bZ/4); \bZ/2) \longrightarrow H^2(\Sp(2g,\bZ/4);\bZ/8). \]
\item[\rm (ix)] We have
\begin{align*}
H^2(\Sp(2g,\bZ);\bZ)&\cong
\begin{cases}\bZ/{12} & \mbox{if }g=1, \\
\bZ \oplus \bZ/2 & \mbox{if }g=2, \\
\bZ & \mbox{if }g\geqslant 3, \end{cases} \\
H^2(\Sp(2g,\bZ);\bZ/8)&\cong\begin{cases}
\bZ/4 & \mbox{if }g=1, \\
\bZ/8 \oplus \bZ/2 \oplus \bZ/2 & \mbox{if }g=2, \\
\bZ/8 \oplus \bZ/2 & \mbox{if }g=3, \\
\bZ/8 & \mbox{if }g\geqslant 4. \end{cases}
\end{align*}
The image of reduction modulo eight is
$\begin{cases}
\bZ/4 & \mbox{if }g=1, \\
\bZ/8 \oplus \bZ/2 & \mbox{if }g=2, \\
\bZ/8 & \mbox{if }g\geqslant 3.\end{cases}$
\item[\rm (x)] For $g \geqslant 3$ the inflation map
\[ H^2(\Sp(2g,\bZ/4); A) \longrightarrow H^2(\Sp(2g,\bZ); A) \]
is injective for any abelian group of coefficients $A$ with trivial action.
\item[\rm (xi)] Pulling back the universal cover of $\Sp(2g,\bR)$ to $\Sp(2g,\bZ)$
gives a group $\widetilde{\Sp(2g,\bZ)}$:
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r] \ar@{=}[d] &
\widetilde{\Sp(2g,\bZ)} \ar[r] \ar[d] & \Sp(2g,\bZ) \ar[r] \ar[d] & 1\\
1 \ar[r] & \bZ \ar[r] & \widetilde{\Sp(2g,\bR)} \ar[r] & \Sp(2g,\bR)
\ar[r] & 1.} \]
This is the universal central extension for $g\geqslant 4$.
For $g=3$, $\Sp(2g,\bbZ{2})$ has an exceptional double cover,
and the pullback of $\widetilde{\Sp(2g,\bZ)}$ %\todo[inline]{$\widetilde{\Sp(2g,\bZ)}$ or $\widetilde{\Sp(2g,\bR)}$?}
and this
double cover over $\Sp(2g, \bZ/2)$ gives the universal central extension of $\Sp(2g,\bZ)$,
with kernel $\bZ \times \bbZ{2}$.


For $g\leqslant 2$, $\Sp(2g,\bZ)$ is not perfect, so it does not have a
universal central extension. But for $g=2$ the cohomology class
defined by the pullback is a generator for a $\bZ$ summand of
$H^2(\Sp(4,\bZ);\bZ)\cong \bZ\oplus \bZ/2$. For $g=1$ the cohomology class
defined by the pullback is a generator for $H^2(\Sp(2,\bZ);\bZ)\cong\bZ/{12}$.
\item[\rm (xii)]The Meyer cocycle
 is four times the generator of $H^2(\Sp(2g,\bZ);\bZ)\cong \bZ$ for
 $g\geqslant 3$, four times the generator for the $\bZ$ summand for
 $g=2$, and an element of order three in $H^2(\Sp(2,\bZ);\bZ)\cong\bZ/{12}$ for $g=1$.
\item[\rm (xiii)] Following the non-zero cohomology class in $H^2(\fH;\bZ/2)$
corresponding to the central extension given in {\rm (v)}
through the maps described in {\rm (vi)--(x)}
\[ H^2(\fH;\bZ/2) \longrightarrow H^2(\Sp(2g,\bZ/4);\bZ/2) \longrightarrow H^2(\Sp(2g,\bZ/4);\bZ/8) \longrightarrow H^2(\Sp(2g,\bZ);\bZ/8) \]
gives the image of the Meyer cohomology class under reduction modulo eight
\[ H^2(\Sp(2g,\bZ);\bZ) \longrightarrow H^2(\Sp(2g,\bZ);\bZ/8) \]
provided $g\geqslant 2$.
Following it through
\[ H^2(\fH;\bZ/2) \longrightarrow H^2(\Sp(2g,\bZ/4);\bZ/2)\longrightarrow H^2(\Sp(2g,\bZ);\bZ/2) \]
gives the image of one quarter of the Meyer cohomology class under
reduction modulo two for $g\geqslant 1$.
\end{enumerate}
\end{theorem}
\begin{proof}
\begin{enumerate}
\item[\rm (i)] See \cite[Theorem 2.2, (i)]{BensonCampagnoloRanickiRovi:2017a}.
\medskip

\item[\rm (ii)] See \cite[Theorem 2.2, (ii)]{BensonCampagnoloRanickiRovi:2017a}.
\medskip


\item[\rm (iii)] The left diagram holds by definition of the groups in presence.

The upper left sequence of the right diagram is already in the left one. The upper right one is to be found in \cite[after Theorem 5.1]{BensonCampagnoloRanickiRovi:2017a}. Note that this shows that $\fsp(2g,\bbZ{2})\cong \Gamma(2g,2)/\Gamma(2g,4)$. This observation proves the exactness of the lower left sequence as well. The lower right one holds by the third isomorphism theorem for groups. The right triangle commutes: it is a composition of quotient maps. The left one commutes as well: it is a composition of inclusions, by definition of $\fY$ and using $\fsp(2g,\bbZ{2})\cong \Gamma(2g,2)/\Gamma(2g,4)$. The square commutes:
$$
\xymatrix
{
\Gamma(2g,2)/\Gamma(2g,4)\ar@{^{(}->}[r]\ar[d]_{/\fK/\Gamma(2g, 4)}&\Sp(2g,\bZ)/(\Gamma(2g, 4)\ar[d]^{/\fK/\Gamma(2g, 4)}\\
\Gamma(2g,2)/\fK\ar@{^{(}->}[r]&\Sp(2g,\bZ)/\fK.
}
$$

\medskip


\item[\rm (iv)]  See \cite[Theorem 2.2, (iii)]{BensonCampagnoloRanickiRovi:2017a} for the claim on the extension.

For the order of $\Sp(2g,\bZ/2)$, see \cite[2.3]{atlas}. For the order of $\fH$, combine the order of $\Sp(2g,\bZ/2)$ with the short exact sequence in the diagram on the right of (iii). The order of $\fsp(2g, \bZ/2)$ is given in \cite[Theorem 5.1]{BensonCampagnoloRanickiRovi:2017a}. Using again the diagrams of (iii), we obtain successively $|\fY|$ and $|\Sp(2g, \bZ/4)|$.
\item[\rm (v)] The existence of the non-trivial double cover of $\fH$ is implied by \cite[Theorem 6.12, Corollary 6.14]{BensonCampagnoloRanickiRovi:2017a} for $g\geq 3$ and by the cohomology group tables in \cite{BensonCampagnoloRanickiRovi:2017a} for $g=1, 2$.

By definition, an almost extraspecial group of order $2^{2g+2}$ is a central product of $\bZ/4$ with an extraspecial group of order $2^{2g+1}$. Its center is a copy of $\bZ/4$.

Griess \cite[Theorem 5 (b)]{Griess:1973a} (see also \cite[Section 3]{BensonCampagnoloRanickiRovi:2017a}) shows that the group $\tilde\fH$ is an extension of $\Sp(2g, \bZ/2)$ by an almost extraspecial group of order $2^{2g+2}$, that we denote by $E$, and that $\tilde\fH/Z(\tilde\fH)$ is isomorphic to the subgroup of index $2$ in $\Aut(E)$ that centralizes the center of $E$. Moreover $Z(\tilde\fH)=Z(E)$ (caveat: the statement in Griess's theorem that says $Z(2^{2g+1})=Z(\tilde\fH)$ is wrong, but his proof shows the correct assertion).

The isomorphism $\tilde\fH/Z(\tilde\fH)\stackrel{\cong}{\rightarrow}\fH/Z(\fH)$ follows from the fact that the preimage of $Z(\fH)$ is exactly $Z(\tilde\fH)$: indeed $|Z(\tilde\fH)|=4$, and $Z(\tilde\fH)$ maps to $Z(\fH)$ with kernel $\bZ/2$.

To see that $|Z(\fH)|$ is (at least) $2$, proceed as follows: the action by conjugation of $\Sp(2g, \bZ/2)$ on the kernel of the extension $(\bZ/2)^{2g+1}$ is trivial for exactly all elements of $\Sp(2g, \bZ/2)$ that lift to an element of $Z(\fH)$. Recall that the action is given through the isomorphism $\Sp(2g, \bZ/2)\cong \Orth(2g+1, \bZ/2)$ \cite[before Remark 5.3]{BensonCampagnoloRanickiRovi:2017a}. The elements that act trivially are therefore the ones lying in the radical of the bilinear form. This is one dimensional, isomorphic to $\bZ/2$.

The commutative braid of extensions is implied by \cite[Theorem 2.2, (ix)]{BensonCampagnoloRanickiRovi:2017a}. %that also states that $E$ is almost extraspecial of the right order. By definition, the group $E$ is then a central product of $\bZ/4$ with an extraspecial group of order $2^{2g+1}$; moreover the conjugation action of $\tilde\fH$
%on $E$ induces an isomorphism between $\tilde\fH/Z(\tilde\fH)$
%and the index two subgroup of
%$\Aut(E)$ centralising $Z(E)$ (see for example \cite[Section 3]{BensonCampagnoloRanickiRovi:2017a} or the original reference by Griess \cite[Theorem 5 (b)]{Griess:1973a}). The assertion about the centers can be checked as follows: Griess \cite[Theorem 5 (b)]{Griess:1973a} states that $Z(\tilde\fH)=Z(2^{2g+1})$, and one can verify by the definition of the central product that................\todo{}

Commutativity of the diagram implies that $\tilde{\fH}$ is non-split as an extension of $\Sp(2g, \bbZ{2})$: the existence of a section of $\tilde\fH\rightarrow \Sp(2g, \bZ/2)$ would imply the existence of a section of $\fH\rightarrow \Sp(2g, \bZ/2)$, and this would contradict (iv).

If $g=1, 2$, then there is more than one isomorphism class of groups $\fH$, and thus $\tilde{\fH}$, fitting in this diagram. The particular group $\fH$ described here is one candidate. This can be checked using the representation of the double cover $\tilde{\fH}$ given in \cite{Benson:theta}.

%\todo[inline, size=\small]{$g=1, 2$? Mail of Dave, 22.9.18}
\item[\rm (vi)] \cite[Corollary 6.14] {BensonCampagnoloRanickiRovi:2017a} and \cite[Corollary 6.5]{BensonCampagnoloRanickiRovi:2017a} imply the inflation of the class corresponding to $\tilde{\fH}$ to a non-zero class in $H^2(\Sp(2g, \bbZ{4}); \bbZ{2})$ and in $H^2(\Sp(2g, \bZ); \bbZ{2})$ for $g\geq 3$.
For $g=1, 2$, the inflation of the class of $\tilde{\fH}$ to non-zero classes in $H^2(\Sp(4, \bbZ{4}); \bbZ{2})$ and in $H^2(\Sp(4, \bZ); \bbZ{2})$ can be taken from the second statement of (xiii) below.

The further inflation to a non-zero class in $H^2(\Gamma_g; \bZ/2)$ follows from the isomorphism $H^2(\Sp(2g, \bZ); \bZ/2)\cong H^2(\Gamma_g; \bZ/2)$ for $g\neq 2$ (see Lemma \ref{Lemma:co-homology computations}\ref{H^2 map Gamma_g Sp Z/2}, which also shows that the statement does not hold for $g=2$).

The braid of extensions describes the groups in presence.

\item[\rm (vii)] See \cite[Corollary 6.14]{BensonCampagnoloRanickiRovi:2017a} for the isomorphism when $g\geq 3$ and \cite[Theorem 6.12]{BensonCampagnoloRanickiRovi:2017a} for the value of $H^2(\fH; \bZ/2)$ for $g=3$. %The statement also appears in \cite[Theorem 2.2, (vii)] {BensonCampagnoloRanickiRovi:2017a}.
Let us recall the argument to obtain the cases $g=1, 2$.

The five-term homology exact sequence associated with 
$$1\longrightarrow \Gamma(2g, 2^n)\longrightarrow \Sp(2g,\bZ)\longrightarrow \Sp(2g,\bZ/2^n)\longrightarrow 1$$
is
\begin{multline*}
H_2(\Sp(2g,\bZ); \bZ)\longrightarrow H_2(\Sp(2g, \bZ/2^n); \bZ)\longrightarrow H_0(\Sp(2g, \bZ/2^n); H_1(\Gamma(2g, 2^n)))\\
\longrightarrow H_1(\Sp(2g,\bZ); \bZ)\longrightarrow H_1(\Sp(2g, \bZ/2^n); \bZ)\longrightarrow 0.
\end{multline*}
By \cite[Lemma 6.2]{BensonCampagnoloRanickiRovi:2017a}, we have $ H_0(\Sp(2g, \bZ/2^n); H_1(\Gamma(2g, 2^n)))=0$ for $g\geq 2, n\geq 1$. %An elementary calculation shows that $H_0(\Sp(2g, \bZ/2^n); H_1(\Gamma(2g, 2^n)))=\bZ/2$ for $g=1, n\geq 1$.
So for every $g\geq 2, n\geq 1$, the map $H_2(\Sp(2g,\bZ); \bZ)\rightarrow H_2(\Sp(2g, \bZ/2^n); \bZ)$ is surjective.% for $g\geq 2$.
% and has cokernel $\bZ/2$ for $g=1$.

The five-term homology exact sequence associated with 
$$1\longrightarrow\fY\longrightarrow\Sp(2g,\bZ/4)\longrightarrow\fH\longrightarrow1$$
is
\begin{multline*}
H_2(\Sp(2g,\bZ/4); \bZ)\longrightarrow H_2(\fH; \bZ)\longrightarrow H_0(\fH; H_1(\fY))\\
\longrightarrow H_1(\Sp(2g,\bZ/4); \bZ)\longrightarrow H_1(\fH; \bZ)\longrightarrow 0.
\end{multline*}
By \cite[Lemma 5.5 i) and proof of Proposition 6.6]{BensonCampagnoloRanickiRovi:2017a} we have $ H_0(\fH; H_1(\fY))=0$ for $g\geq 1$. The map $H_2(\Sp(2g,\bZ/4); \bZ)\rightarrow H_2(\fH; \bZ)$ is thus surjective for $g\geq 1$. Together with the above this implies that $H_2(\Sp(2g,\bZ/2^n); \bZ)\rightarrow H_2(\fH; \bZ)$ is surjective for all $g, n\geq2$.
Consider the sequence of induced maps
$$\mathsf{Hom}(H_2(\Sp(2g,\bZ); \bZ), \bZ/2)\longleftarrow \mathsf{Hom}(H_2(\Sp(2g, \bZ/2^n); \bZ), \bZ/2)\longleftarrow \mathsf{Hom}(H_2(\fH; \bZ), \bZ/2).$$
By the above both are injective for $g, n\geq 2$. % and the second one is also for $g=1$.
Insert the values of $H_2(\Sp(2g,\bZ); \bZ)$ (Lemma \ref{Lemma:co-homology computations}\ref{H_2 Sp Z Z}) and $H_2(\fH; \bZ)$ \cite[Tables]{BensonCampagnoloRanickiRovi:2017a}. We see that both maps must be isomorphisms for $g, n\geq 2$. By the universal coefficient theorem this finishes the proof for $g\geq 3$, as each of $\Sp(2g,\bZ), \Sp(2g, \bZ/2^n)$, and $\fH$ are perfect.

For $g=1, 2$, we need to also consider the $\mathsf{Ext}$-terms coming from $H_1(\Sp(2g,\bZ);\bZ)$, $H_1(\Sp(2g, \bZ/2^n);\bZ)$, and $H_1(\fH; \bZ)$. By the five-term exact sequences above, the maps $H_1(\Sp(2g,\bZ); \bZ)\rightarrow H_1(\Sp(2g, \bZ/2^n)$  for every $n\geq 1$ and $H_1(\Sp(2g,\bZ/4); \bZ)\rightarrow H_1(\fH; \bZ)$ are surjective. This implies that $$H_1(\Sp(2g, \bZ/2^n)\longrightarrow H_1(\fH; \bZ)$$ is surjective for all $n\geq 2$ as well. Insert the values of $H_1(\Sp(2g,\bZ); \bZ)$ (Lemma \ref{Lemma:co-homology computations}\ref{H_1 Sp}) and $H_1(\fH; \bZ)$ \cite[Tables]{BensonCampagnoloRanickiRovi:2017a}.

For $g=2$ the composition 
$$\bZ/2\cong H_1(\Sp(2g,\bZ);\bZ)\longrightarrow H_1(\Sp(2g, \bZ/2^n);\bZ)\longrightarrow H_1(\fH; \bZ)\cong\bZ/2$$
is surjective, thus also injective. Then each of the two maps is an isomorphism, and thus by functoriality we obtain isomorphisms also for 
$$\mathsf{Ext}^1_{\bZ}(H_1(\fH; \bZ), \bZ/2)\longrightarrow \mathsf{Ext}^1_{\bZ}(H_1(\Sp(2g, \bZ/2^n);\bZ), \bZ/2)\longrightarrow \mathsf{Ext}^1_{\bZ}(H_1(\Sp(2g,\bZ);\bZ), \bZ/2)$$
for every $n\geq 2$. This together with the preceding results on the $\mathsf{Hom}$-term finishes the proof for $g=2$.

For $g=1$ the composition 
$$\bZ/12\cong H_1(\Sp(2g,\bZ);\bZ)\longrightarrow H_1(\Sp(2g, \bZ/2^n);\bZ)\longrightarrow H_1(\fH; \bZ)\cong\bZ/4$$
is surjective, thus the middle term is either $\bZ/12$ or $\bZ/4$. For $n=2$ it is $\bZ/4$, as in this case $\fH=\Sp(2, \bZ/4)$ (Point (iv) above). To determine it for $n>2$ we use yet another short exact sequence
$$1\longrightarrow\fsp(2, \bZ/2)\longrightarrow\Sp(2,\bZ/2^{n+1})\longrightarrow\Sp(2, \bZ/2^n)\longrightarrow1$$
(see \cite[before Proposition 5.2]{BensonCampagnoloRanickiRovi:2017a}) and its associated five-term homology exact sequence:
\begin{multline*}
H_2(\Sp(2,\bZ/2^{n+1}); \bZ)\longrightarrow H_2(\Sp(2, \bZ/2^n); \bZ)\longrightarrow H_0(\Sp(2, \bZ/2^n); H_1(\fsp(2, \bZ/2)))\\
\longrightarrow H_1(\Sp(2,\bZ/2^{n+1}); \bZ)\longrightarrow H_1(\Sp(2, \bZ/2^n); \bZ)\longrightarrow 0.
\end{multline*}
Note that $\fsp(2, \bZ/2)\cong(\bZ/2)^{3}$ \cite[Theorem 5.1]{BensonCampagnoloRanickiRovi:2017a}. Therefore $H_1(\fsp(2, \bZ/2))=\fsp(2, \bZ/2)$ and $H_0(\Sp(2, \bZ/2^n); H_1(\fsp(2, \bZ/2)))$ is the coinvariants of the action of $\Sp(2, \bZ/2^n)$, that is some quotient of $(\bZ/2)^3$; in particular it has no $3$-torsion.

Recall as well that $\Sp(2, \bZ/2)\cong\mathrm{Sym}(3)$ and thus $H_1(\Sp(2, \bZ/2); \bZ)=\bZ/2$, $H_2(\Sp(2, \bZ/2); \bZ)=0$ \cite[Tables]{BensonCampagnoloRanickiRovi:2017a}.

Use induction on $n$ to determine the $3$-torsion of $H_1(\Sp(2,\bZ/2^{n+1}); \bZ)$: by the five-term exact sequence and what we just said, it has to be the same as the $3$-torsion of $H_1(\Sp(2, \bZ/2); \bZ)$, which is $0$. Therefore we obtain $H_1(\Sp(2,\bZ/2^{n}); \bZ)\cong\bZ/4$ and the map $H_1(\Sp(2g, \bZ/2^n);\bZ)\rightarrow H_1(\fH; \bZ)$ is an isomorphism for all $n\geq 2$.

Now go back to the five-term exact sequence 
\begin{multline*}
H_2(\Sp(2,\bZ); \bZ)\longrightarrow H_2(\Sp(2, \bZ/2^n); \bZ)\longrightarrow H_0(\Sp(2, \bZ/2^n); H_1(\Gamma(2, 2^n)))\\
\longrightarrow H_1(\Sp(2,\bZ); \bZ)\longrightarrow H_1(\Sp(2, \bZ/2^n); \bZ)\longrightarrow 0.
\end{multline*}
What we know translates into
\begin{multline*}
0\longrightarrow H_2(\Sp(2, \bZ/2^n); \bZ)\longrightarrow H_0(\Sp(2, \bZ/2^n); H_1(\Gamma(2, 2^n)))
\longrightarrow \bZ/12\longrightarrow \bZ/4\longrightarrow 0.
\end{multline*}
We have $H_0(\Sp(2, \bZ/2^n); H_1(\Gamma(2, 2^n)))\cong\bZ/6$. Thus $H_2(\Sp(2, \bZ/2^n); \bZ)\cong\bZ/2$ for all $n\geq 2$.
\todo[inline]{$H_0(\Sp(2, \bZ/2^n); H_1(\Gamma(2, 2^n)))\cong\bZ/6$ for $n\geq 3$? also need a surjection $H_2(\Sp(2,\bZ/2^{n+1}); \bZ)\longrightarrow H_2(\Sp(2, \bZ/2^n); \bZ)$? }

Comparing with the values of $H_1(\fH; \bZ), H_2(\fH; \bZ)$ and using the universal coefficient theorem finishes the proof.
%See more cohomology computations in Lemma  \ref{Lemma:co-homology computations} \ref{H^2 Sp Z/4 Z/2}.
\item[\rm (viii)] (See also \cite[Chapter 6]{CampagnoloThesis}.) We consider the following short exact sequence:
$$
\xymatrix
{
0\ar[r]&\mathbb{Z}/2\ar[r]^{i} & \mathbb{Z}/8\ar[r]^{p} &\mathbb{Z}/4\ar[r]&0,
}
$$ 
where $i$ is the map sending $1$ to $4$.
The induced long exact sequence in cohomology for $\Sp(2g, \mathbb{Z}/4)$ is:
$$\begin{tikzpicture}[descr/.style={fill=white,inner sep=1pt}]
        \matrix (m) [
            matrix of math nodes,
            row sep=1.5em,
            column sep=2.5em,
            text height=1.5ex, text depth=0.25ex
        ]
       {  & ... & H^1(\Sp(2g, \mathbb{Z}/4); \mathbb{Z}/4) \\
             H^2(\Sp(2g, \mathbb{Z}/4); \mathbb{Z}/2) & H^2(\Sp(2g, \mathbb{Z}/4);\mathbb{Z}/8) & H^2(\Sp(2g, \mathbb{Z}/4);\mathbb{Z}/4) \\
            H^3(\Sp(2g, \mathbb{Z}/4);\mathbb{Z}/2) &... & \\
            &     \mbox{}    &                 &      \mbox{}    \\
        };
 \path[overlay,->, font=\scriptsize,>=latex]
        (m-1-2) edge node[descr,yshift=0.3ex] {$p^*$}(m-1-3)
      
       (m-1-3) edge[out=355,in=175] node[descr,yshift=0.3ex] {$\partial^1$} (m-2-1)
        (m-2-1) edge node[descr,yshift=0.3ex] {$i^*$}(m-2-2)
        (m-2-2) edge node[descr,yshift=0.3ex] {$p^*$} (m-2-3)
        (m-2-3) edge[out=355,in=175] node[descr,yshift=0.3ex] {$\partial^2$} (m-3-1)
        (m-3-1) edge node[descr,yshift=0.3ex] {$i^*$} (m-3-2);
\end{tikzpicture}$$
Let $g\geq 3$. Then $H^1(\Sp(2g, \mathbb{Z}/4); \mathbb{Z}/4)=0$ by perfection of the group. Using the cohomology computations of point (vii) and Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp Z/4 Z/8}, we thus have an isomorphism $i^*$
$$H^2(\Sp(2g, \mathbb{Z}/4); \mathbb{Z}/2)\stackrel{\cong}{\longrightarrow} H^2(\Sp(2g, \mathbb{Z}/4);\mathbb{Z}/8).$$
\medskip


\item[\rm (ix)] See Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp Z Z},\ref{H^2 Sp Z Z/8},\ref{H^2 Sp image r8}.
\medskip


\item[\rm (x)] By \cite[Corollary 6.5]{BensonCampagnoloRanickiRovi:2017a}.
\medskip


\item[\rm (xi)] See\cite[Section 1] {BensonCampagnoloRanickiRovi:2017a} for $g\geq 3$.
For $g=1, 2$, consider the following commutative diagram:
$$
\xymatrix
{
 & \bZ\ar[r]& \widetilde{\Sp(8, \bZ)}\ar[r]& \Sp(8, \bZ)\ar[dr] & \\
1\ar[ur]\ar[dr]\ar[r] & \bZ\ar[r]\ar[u]_=& \widetilde{\Sp(4, \bZ)}\ar[r]\ar@{^{(}->}[u]& \Sp(4, \bZ)\ar@{^{(}->}[u]\ar[r] &1 \\
& \bZ\ar[r]\ar[u]_=& \widetilde{\Sp(2, \bZ)}\ar[r]\ar@{^{(}->}[u]& \Sp(2, \bZ)\ar@{^{(}->}[u]\ar[ur] & \\
}
$$
The inclusions of the symplectic groups $\Sp(2, \bZ)\subset\Sp(4, \bZ)\subset\Sp(8, \bZ)$ induce morphisms in cohomology $$
\xymatrix
{
H^2(\Sp(8, \bZ); \bZ)\cong\bZ\ar[r]& H^2(\Sp(4, \bZ); \bZ)\cong\bZ\oplus\bZ/2\ar[r]& H^2(\Sp(2, \bZ); \bZ)\cong\bZ/12
}
$$ that map $[\tau_4]=4\mapsto [\tau_2]=(4, 0)\mapsto[\tau_1]=4\mbox{ or }8$ by Proposition \ref{pr:cocycles-restrict}(ii). For the generators we obtain $1\mapsto (1, 0)\mapsto 1, 5, 7 \mbox{ or }11\in\bZ/12$ (see Lemma \ref{lemma: genSp8toSp2} and also the proof of Point (xii) below). This proves the statement for $g=1, 2$.
%\todo{Is the image of $c_1$ in $H^2(\Sp(2, \bZ), \bZ)$ a generator?}

\medskip


\item[\rm (xii)]%See \cite[Satz 2]{Meyer:1973a} for $g=1$, as in this case we have $\Gamma_1=\Sp(2, \bZ)$, and also for $g\geq 3$ as the map $p^*:H^2(\Sp(2g, \bZ), \bZ)\rightarrow H^2(\Gamma_g, \bZ)$ is an isomorphism (see \ref{H^2 map Gamma_g Sp} in Lemma \ref{Lemma:co-homology computations}). Moreover in \cite[p. 244]{Meyer:1973a} Meyer computes the restriction of his cocycle $[\tau_g]$ to subgroups of the form $\Sp(2g_1, \bZ)\times...\times\Sp(2g_r, \bZ)\stackrel{j}{\hookrightarrow} \Sp(2g, \bZ)$, with $\sum_{i=1}^{r}g_i=g$, and shows that
%$$j^*\tau_g((\alpha_1, ...\alpha_r), (\beta_1, ..., \beta_r))=\sum_{i=1}^{r}\tau_{g_i}(\alpha_i, \beta_i).$$
%Now consider the commutative diagram
%$$
%\xymatrix
%{
%\bZ\cong H^2_b(\Sp(6, \bR), \bZ)\ar[r]^{\cong}\ar[d]^{\cong}&H^2(\Sp(6, \bZ), \bZ)\cong\bZ\ar[d]^{j^*}\\
%\bZ\cong H^2_b(\Sp(4, \bR), \bZ)\ar@{^{(}->}[r]&H^2(\Sp(4, \bZ), \bZ)\cong\bZ\oplus\bZ/2.
%}
%$$
%The vertical isomorphism comes from Corollary \ref{co:H_b^2Sp} while the horizontal one is given by \cite[Proposition 3.1, p. 258]{barge-ghys}, as the groups in presence are cyclic (see also the proof of Lemma \ref{Lemma:co-homology computations}\ref{H_2 map Gamma_g Sp}). The injection at the bottom comes from the same argument: the first Chern class $c_1$ is sent to $\frac{1}{4}[\tau_3]$ in the top line, and to either $(\frac{1}{4}[\tau_2], 0)$ or $(\frac{1}{4}[\tau_2], 1)\in\bZ\oplus\bZ/2$ in the bottom line. But now $j^*$, with $g_1=2, g_2=1, g=3$, further restricted to $\alpha_2=\beta_2=\mathrm{id}$, shows that it is $(\frac{1}{4}[\tau_2], 0)$, just as claimed. 

See \cite[Satz 2]{Meyer:1973a} for $g=1$, as in this case we have $\Gamma_1=\Sp(2, \bZ)$, and also for $g\geq 3$ as the map $p^*\colon H^2(\Sp(2g, \bZ); \bZ)\rightarrow H^2(\Gamma_g; \bZ)$ is an isomorphism (see Lemma \ref{Lemma:co-homology computations}\ref{H^2 map Gamma_g Sp}). For $g=2$, consider the commutative diagram
$$
\xymatrix
{
\bZ\cong H^2_b(\Sp(6, \bR); \bZ)\ar[r]^{\cong}\ar[d]^{\cong}_r&H^2(\Sp(6, \bZ); \bZ)\cong\bZ\ar[d]^{r_\bZ}\\
\bZ\cong H^2_b(\Sp(4, \bR); \bZ)\ar@{^{(}->}[r]&H^2(\Sp(4, \bZ); \bZ)\cong\bZ\oplus\bZ/2.
}
$$
The map $r$ is an isomorphism by Corollary \ref{co:H_b^2Sp}, while the horizontal isomorphism is given by \cite[Proposition 3.1, p. 258]{barge-ghys}, as the groups in presence are cyclic (see also the proof of Lemma \ref{Lemma:co-homology computations}\ref{H_2 map Gamma_g Sp}). The injection at the bottom comes from the same argument: the first Chern class $c_1$ is sent to $\frac{1}{4}[\tau_3]$ in the top line, and to either $(\frac{1}{4}[\tau_2], 0)$ or $(\frac{1}{4}[\tau_2], 1)\in\bZ\oplus\bZ/2$ in the bottom line. But Proposition \ref{pr:cocycles-restrict}(ii) says that the map $r$ sends $\tau_3$ to $\tau_2$ even as cocycles; a fortiori this is true for $r_\bZ$ on the restrictions of $\tau_3$ and $\tau_2$. So composing the arrrows shows that $c_1$ goes to $(\frac{1}{4}[\tau_2], 0)$, just as claimed.
%For $g=2$, Meyer states that it has infinite order (see \cite[p. 263]{Meyer:1973a})
\item[\rm (xiii)] For $g\geq 4$, the first statement is obtained as follows: denote by $[\eta]\in H^2(\fH; \bbZ{2})$ the generator corresponding to the extension $\tilde{\fH}$. The first map is an isomorphism by (vii), the second  by (viii), the third is injective by (x), so that, using the computations in (vii) and (ix) the image of $[\eta]$ in $H^2(\Sp(2g, \bZ); \bbZ{8})$ is $4\in \bbZ{8}$. By (ix) again, this is exactly the image of $[\tau_g]=4\in H^2(\Sp(2g, \bZ); \bZ)$ in $H^2(\Sp(2g, \bZ); \bbZ{8})$.

For $g=3$, consider the following commutative diagram:

{\footnotesize
$$
\xymatrix
{ 
\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/8\oplus\bZ/2\ar[d]^{\cong}& \bZ\ar[d]^{\cong}\\
H^2(\fH; \bZ/2)\ar[r] & H^2(\Sp(6, \bZ/4); \bZ/2)\ar[r]& H^2(\Sp(6, \bZ/4); \bZ/8)\ar[r]& H^2(\Sp(6, \bZ); \bZ/8)&H^2(\Sp(6, \bZ); \bZ)\ar[l]\\
H^2(\fH; \bZ/2)\ar[r]_-{\cong}\ar[u]_f & H^2(\Sp(8, \bZ/4); \bZ/2)\ar[r]_{\cong}\ar[u]_h& H^2(\Sp(8, \bZ/4); \bZ/8)\ar@{^{(}->}[r]\ar[u]_k& H^2(\Sp(8, \bZ); \bZ/8)\ar[u]_\ell&H^2(\Sp(8, \bZ); \bZ)\ar[l]\ar[u]_{\cong}\\
\bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}& \bZ/8\ar[u]_{\cong}& \bZ\ar[u]_{\cong}
}
$$ }
The class $[\tau_4]\in H^2(\Sp(8, \bZ); \bZ)$ maps to $[\tau_3]\in H^2(\Sp(6, \bZ); \bZ)$ by Proposition \ref{pr:cocycles-restrict}(ii) and to $4\in H^2(\Sp(8, \bZ); \bZ/8)\cong\bZ/8$ by (ix). By (ix) again, $[\tau_3]$ maps to $(4, 0)\in\bZ/8\oplus\bZ/2$. The map $\ell$ is thus injective. Then $k$ has to be injective too, and so does $h$, and then $f$. Consequently, the non-zero class $f([\eta])$ is mapped under composition of the maps in the first line of the diagram to $\ell(4)=(4, 0)\in H^2(\Sp(6, \bZ); \bZ/8)$. As we remarked, this is the image of $[\tau_3]$ in $H^2(\Sp(6, \bZ); \bZ/8)$. That proves the first statement for $g=3$.

For $g=2$, we reason in the same way. We have the following commutative diagram:
{ \footnotesize
$$
\xymatrix
{
& \bZ/2\oplus\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/8\oplus\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ\oplus\bZ/2\ar[d]^{\cong}\\
H^2(\fH; \bZ/2)\ar[r] & H^2(\Sp(4, \bZ/4); \bZ/2)\ar[r]& H^2(\Sp(4, \bZ/4); \bZ/8)\ar[r]& H^2(\Sp(4, \bZ); \bZ/8)&H^2(\Sp(4, \bZ); \bZ)\ar[l]\\
H^2(\fH; \bZ/2)\ar[r]_-{\cong}\ar[u]_f & H^2(\Sp(8, \bZ/4); \bZ/2)\ar[r]_{\cong}\ar[u]_h& H^2(\Sp(8, \bZ/4); \bZ/8)\ar@{^{(}->}[r]\ar[u]_k& H^2(\Sp(8, \bZ); \bZ/8)\ar[u]_\ell&H^2(\Sp(8, \bZ); \bZ)\ar[l]\ar@{^{(}->}[u]\\
\bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}& \bZ/8\ar[u]_{\cong}& \bZ\ar[u]_{\cong}
}
$$ }
The class $[\tau_4]\in H^2(\Sp(8, \bZ); \bZ)$ maps to $[\tau_2]\in H^2(\Sp(4, \bZ); \bZ)$ by Proposition \ref{pr:cocycles-restrict}(ii) and to $4\in H^2(\Sp(8, \bZ); \bZ/8)\cong\bZ/8$ by (ix). By (ix) again, $[\tau_2]$ maps to $(4, 0, 0)\in\bZ/8\oplus\bZ/2\oplus\bZ/2$. The map $\ell$ is thus injective. Then $k$ has to be injective too, and so does $h$, and then $f$. Consequently, the non-zero class $f([\eta])$ is mapped under composition of the maps in the first line of the diagram to $\ell(4)=(4, 0, 0)\in H^2(\Sp(4, \bZ); \bZ/8)$. As we remarked, this is the image of $[\tau_2]$ in $H^2(\Sp(4, \bZ); \bZ/8)$. That proves the first statement for $g=2$.

The second statement follows from \cite[Theorem 2.2, (viii)]{BensonCampagnoloRanickiRovi:2017a} for $g\geq 4$.

For $g=3$, consider the following commutative diagram:
$$
\xymatrix
{ 
\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ\ar[d]^{\cong}\\
H^2(\fH; \bZ/2)\ar[r] & H^2(\Sp(6, \bZ/4); \bZ/2)\ar[r]& H^2(\Sp(6, \bZ); \bZ/2)&H^2(\Sp(6, \bZ); \bZ)\ar[l]\\
H^2(\fH; \bZ/2)\ar[r]_-{\cong}\ar[u]_f & H^2(\Sp(8, \bZ/4); \bZ/2)\ar[r]_{\cong}\ar[u]_h& H^2(\Sp(8, \bZ); \bZ/2)\ar[u]_\ell&H^2(\Sp(8, \bZ); \bZ)\ar[l]\ar[u]_{\cong}\\
\bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}&  \bZ/2\ar[u]_{\cong}& \bZ\ar[u]_{\cong}
}
$$
The class $1\in H^2(\Sp(8, \bZ); \bZ)$ maps to $1\in H^2(\Sp(6, \bZ); \bZ)$ by Proposition \ref{pr:cocycles-restrict}(ii) and to $1\in H^2(\Sp(8, \bZ); \bZ/2)\cong\bZ/2$ by Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2}. By Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2} again, $1$ maps to $(1, 0)\in H^2(\Sp(6, \bZ); \bZ/2)\cong\bZ/2\oplus\bZ/2$. The map $\ell$ is thus injective. Then $h$ has to be injective too, and so does $f$. Consequently, the non-zero class $f([\eta])$ is mapped under composition of the maps in the first line of the diagram to $\ell(1)=(1, 0)\in H^2(\Sp(6, \bZ); \bZ/2)$. As we remarked, this is the image of $1\in H^2(\Sp(6, \bZ); \bZ)$ in $H^2(\Sp(6, \bZ); \bZ/2)$. That proves the second statement for $g=3$.

For $g=2$, we reason in the same way. We have the following commutative diagram:
$$
\xymatrix
{ 
& \bZ/2\oplus\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\oplus\bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ\oplus\bZ/2\ar[d]^{\cong}\\
H^2(\fH; \bZ/2)\ar[r] & H^2(\Sp(4, \bZ/4); \bZ/2)\ar[r]& H^2(\Sp(4, \bZ); \bZ/2)&H^2(\Sp(4, \bZ); \bZ)\ar[l]\\
H^2(\fH; \bZ/2)\ar[r]_-{\cong}\ar[u]_f & H^2(\Sp(8, \bZ/4); \bZ/2)\ar[r]_{\cong}\ar[u]_h& H^2(\Sp(8, \bZ); \bZ/2)\ar[u]_\ell&H^2(\Sp(8, \bZ); \bZ)\ar[l]\ar@{^{(}->}[u]\\
\bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}&  \bZ/2\ar[u]_{\cong}& \bZ\ar[u]_{\cong}
}
$$
The class $1\in H^2(\Sp(8, \bZ); \bZ)$ maps to $(1, 0)\in H^2(\Sp(4, \bZ); \bZ)$ by Proposition \ref{pr:cocycles-restrict}(ii) (see also the proof of (xii) above) and to $1\in H^2(\Sp(8, \bZ); \bZ/2)\cong\bZ/2$ by Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2}. By Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2} again, $(1, 0)$ maps to $(1, 0, 0)\in H^2(\Sp(4, \bZ); \bZ/2)\cong\bZ/2\oplus\bZ/2\oplus\bZ/2$. The map $\ell$ is thus injective. Then $h$ has to be injective too, and so does $f$. Consequently, the non-zero class $f([\eta])$ is mapped under composition of the maps in the first line of the diagram to $\ell(1)=(1, 0, 0)\in H^2(\Sp(4, \bZ); \bZ/2)$. As we remarked, this is the image of $(1, 0)\in H^2(\Sp(4, \bZ); \bZ)$ in $H^2(\Sp(4, \bZ); \bZ/2)$. That proves the second statement for $g=2$.

For $g=1$, we use the same method:
$$
\xymatrix
{ 
& \bZ/2\oplus\bZ/2\ar[d]^{\cong}& \bZ/2\ar[d]^{\cong}& \bZ/12\ar[d]^{\cong}\\
H^2(\fH; \bZ/2)\ar[r]^-{=}& H^2(\Sp(2, \bZ/4); \bZ/2)\ar[r]& H^2(\Sp(2, \bZ); \bZ/2)&H^2(\Sp(2, \bZ); \bZ)\ar[l]\\
H^2(\fH; \bZ/2)\ar[r]_-{\cong}\ar[u]_f & H^2(\Sp(8, \bZ/4); \bZ/2)\ar[r]_{\cong}\ar[u]_h& H^2(\Sp(8, \bZ); \bZ/2)\ar[u]_\ell&H^2(\Sp(8, \bZ); \bZ)\ar[l]\ar[u]\\
\bZ/2\ar[u]_{\cong}& \bZ/2\ar[u]_{\cong}&  \bZ/2\ar[u]_{\cong}& \bZ\ar[u]_{\cong}
}
$$

The class $1\in H^2(\Sp(8, \bZ); \bZ)$ maps to $1, 5 , 7\mbox{ or } 11$ by Lemma \ref{lemma: genSp8toSp2} and to $1\in H^2(\Sp(8, \bZ); \bZ/2)\cong\bZ/2$ by Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2}. By Lemma \ref{Lemma:co-homology computations}\ref{H^2 Sp image r2} again, $1, 5, 7\mbox{ or } 11\in\bZ/12$ maps to $1\in H^2(\Sp(2, \bZ); \bZ/2)\cong\bZ/2$. The map $\ell$ is thus injective. Then $h$ has to be injective too, and so does $f$. Consequently, the non-zero class $f([\eta])$ is mapped under composition of the maps in the first line of the diagram to $\ell(1)=1\in H^2(\Sp(2, \bZ); \bZ/2)$. As we remarked, this is the image of $1, 5 , 7\mbox{ or } 11\in H^2(\Sp(2, \bZ); \bZ)$ in $H^2(\Sp(2, \bZ); \bZ/2)$. That proves the second statement for $g=1$.
\end{enumerate}
\end{proof}
The following diagram, valid for $g\geqslant 4$, may help clarify the theorem.
\[ \xymatrix@=8mm{
\bZ/2=H^2(\fH;\bZ/2) \ar[r]^\cong \ar[d]^\cong &
H^2(\fH;\bZ/8)=\bZ/2 \ar[d]^\cong \\
\bZ/2=H^2(\Sp(2g,\bZ/4);\bZ/2) \ar[r]^\cong \ar[d]^\cong &
H^2(\Sp(2g,\bZ/4);\bZ/8)=\bZ/2 \ar[d]^4 \\
\bZ/2=H^2(\Sp(2g,\bZ);\bZ/2) \ar[r]^4 &
H^2(\Sp(2g,\bZ);\bZ/8)=\bZ/8 \\
\bZ=H^2(\Sp(2g,\bZ);\bZ) \ar[r]^4 \ar@{->>}[u] &
H^2(\Sp(2g,\bZ);\bZ)=\bZ \ar@{->>}[u]} \]
This illustrates the connection between Meyer's cohomology class on the bottom
right and the central extension $\tilde \fH$ of $\fH$ regarded as a cohomology class on the top left.


\subsection{Signatures of surface bundles mod $N$ for $N>8$}\label{Signatures of surface bundles mod $N$ for $N>8$}


We just explained the existence of a cohomology class in the second cohomology group of the finite quotient $\fH$ of $\Sp(2g, \bZ)$ that computes the mod 2 reduction of signature/4 for a surface bundle over a surface. Here we explain in detail why this information on the signature is the best we can hope for if we restrict ourselves to cohomology classes on finite quotients of the symplectic group.

Precisely, we want to show the following:
\begin{theorem}\label{cas Z/m}
Let $g\geqslant 4$ and $K\leq \Sp(2g, \bZ)$ be a normal subgroup of finite index. %in $\mathrm{Sp}(2g, \bZ)$.
If $c \in H^2(\Sp(2g,\bZ)/K;\bZ/N)$ is a cohomology class such that for the monodromy $\bar\chi\colon\pi_1(\Sigma_h)\rightarrow\Sp(2g,\bZ)$ of any surface bundle $\Sigma_g\rightarrow E\rightarrow\Sigma_h$ we have $$\sigma(E) = -\langle\bar\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/N,$$
%and $\langle\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/m$ is not constant equal to $0$
then $N=2, 4,$ or $8$. If $N=2$ or $4$, the value $\langle\bar\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/N$ is always $0$. Here $p\colon\Sp(2g,\bZ)\rightarrow\Sp(2g,\bZ)/K$ denotes the quotient map.
\end{theorem}
This will be a direct consequence of a more general result (see also Remark \ref{Z/m}):
\begin{theorem}\label{cas general}
Let $g\geqslant 4$ and $K\leq \Sp(2g, \bZ)$ be a normal subgroup of finite index, and $A$ be a commutative ring. If $c \in H^2(\Sp(2g,\bZ)/K; A)$ is a cohomology class such that for the monodromy $\bar\chi\colon\pi_1(\Sigma_h)\rightarrow\Sp(2g,\bZ)$ of any surface bundle $\Sigma_g\rightarrow E\rightarrow\Sigma_h$ we have $$\sigma(E) = -\langle\bar\chi^*p^*(c),[\Sigma_h]\rangle \in A,$$
then $\langle\bar\chi^*p^*(c),[\Sigma_h]\rangle$ is the image of $4\in\bZ$ in $A$ and lies in the $2$-torsion of $A$. Here $p\colon\Sp(2g,\bZ)\rightarrow\Sp(2g,\bZ)/K$ denotes the quotient map.%From the second cohomology of any finite quotient of $\mathrm{Sp}(2g, \bZ)$ with coefficients in any principal ideal domain $A$ one cannot recover more information on the signature of a surface bundle over a surface than a $2$-valued homomorphic image.
\end{theorem}
Morally, this theorem says that any cohomology class on a finite quotient of the symplectic group yields at most a $2$-valued information on the signature of a surface bundle over a surface (as it lies in the $2$-torsion of the arbitrary coefficient ring $A$).

The above results rely on the non-residual finiteness of $\widetilde{\Sp(2g, \bZ)}$  proved by Deligne \cite{Deligne:1978a}. We recall the setup.

Let $\widetilde{\Sp(2g, \bZ)}$ denote the central extension obtained by pulling back the universal cover of $\Sp(2g, \mathbb{R})$ to $\Sp(2g, \bZ)$:
$$\xymatrix{
1\ar[r]&\bZ\ar[r]\ar@{=}[d]&\widetilde{\Sp(2g, \bZ)}\ar[r]_u\ar[d]&\Sp(2g, \bZ)\ar[r]\ar[d]&1\phantom{.}\\
1\ar[r]&\bZ\ar[r]&\widetilde{\Sp(2g, \mathbb{R})}\ar[r]&\Sp(2g, \mathbb{R})\ar[r]&1.
}$$
For $g\geqslant 4$, the group $\widetilde{\Sp(2g, \bZ)}$ is the universal central extension of the perfect group $\Sp(2g, \bZ)$.

Let $[\tau_g]\in H^2(\Sp(2g, \bZ); \bZ)$ denote the class of the Meyer signature cocycle. Recall that $[\tau_g]=4\in\bZ\cong H^2(\Sp(2g, \bZ); \bZ)$ for $g\geqslant 3$.
\begin{theorem}[Deligne \cite{Deligne:1978a}]\label{deligne}
For $g\geqslant 2$, the group $\widetilde{\Sp(2g, \bZ)}$ is not residually finite: every subgroup of finite index contains the subgroup $2\bZ$.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{cas general}]
Let $Q=\Sp(2g,\bZ)/K$ be a finite quotient of $\Sp(2g, \bZ)$. Denote by $p\colon\Sp(2g,\bZ)\rightarrow Q$ the projection map. We have a natural isomorphism 
$$\begin{array}{ccc}
\widetilde{\Sp(2g, \bZ)}/\widetilde{K}&\longrightarrow &\Sp(2g, \bZ)/K\\
\widetilde{g}\widetilde{K}&\longmapsto &u(\tilde{g})K,
\end{array}$$
where $\widetilde{K}=u^{-1}(K)$ denotes the preimage of $K$ in $\widetilde{\Sp(2g, \bZ)}$. So $[\widetilde{\Sp(2g, \bZ)}:\widetilde{K}]<\infty$. By Theorem \ref{deligne}, the subgroup $\widetilde{K}$ then contains $2\bZ$.

Note that as $\widetilde{\Sp(2g, \bZ)}$ is the universal central extension of $\Sp(2g, \bZ)$ for $g\geqslant 4$, the central subgroup of the extension is isomorphic to the second homology group:
$$\bZ\cong H_2(\Sp(2g, \bZ); \bZ),\, \forall g\geqslant 4.$$
%For $g=3$, we have
%$$\bZ\oplus\bZ/2\bZ\cong H_2(\mathrm{Sp}(2g, \bZ), \bZ).$$

{\bfseries Claim 1:} The map induced by $p$ in homology annihilates the subgroup $2\bZ$:
$$2\bZ\leq \mathsf{ker}\left(p_*\colon H_2(\Sp(2g, \bZ); \bZ)\longrightarrow H_2(Q; \bZ)\right).$$

{\bfseries Proof of Claim 1:} As a quotient of the perfect group $\Sp(2g, \bZ)$, the group $Q$ is perfect. Hence it possesses a universal central extension $\widetilde{Q}$ satisfying:
$$\xymatrix{
1\ar[r]&H_2(Q; \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1.
}$$
Denote by $E$ the pullback of $\widetilde{Q}$ and $\Sp(2g, \bZ)$ fitting in the following comutative diagram:
$$\xymatrix{
1\ar[r]&H_2(Q; \bZ)\times\{\mathrm{id}\}\ar[r]\ar[d]_{p_1}& E\ar[d]_{p_1}\ar[r]_-{p_2}& \Sp(2g, \bZ)\ar[r]\ar[d]_p&1\phantom{.}\\
1\ar[r]&H_2(Q; \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1.
}$$
The maps $p_1$ and $p_2$ denote the projections to the first and the second factor respectively, and $$E=\left\{(\tilde{q}, g)\in\widetilde{Q}\times\Sp(2g, \bZ)\,\vline\, \pi(\tilde{q})=p(g)\right\}.$$
They are both surjective, as $\pi$ and $p$ are. Moreover one checks directly that $E$ is a central extension of $\Sp(2g, \bZ)$. Consequently by the properties of the universal central extension, there exists a unique map $\phi\colon \widetilde{\Sp(2g, \bZ)}\rightarrow E$ such that $p_2\circ\phi=u$. We now have the commutative diagram
$$\xymatrix{
1\ar[r]&H_2(\Sp(2g, \bZ); \bZ)\ar[r]\ar[d]_{\phi}& \widetilde{\Sp(2g, \bZ)}\ar[d]_{\phi}\ar[dr]^-{u}&&\\
1\ar[r]&H_2(Q; \bZ)\times\{\mathrm{id}\}\ar[r]\ar[d]_{p_1}& E\ar[d]_{p_1}\ar[r]_-{p_2}& \Sp(2g, \bZ)\ar[r]\ar[d]_p&1\phantom{.}\\
1\ar[r]&H_2(Q; \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1.
}$$
By functoriality (and general knowledge on the second homology of perfect groups) the leftmost composition $p_1\circ\phi$ is precisely the induced map in homology $p_*\colon H_2(\Sp(2g, \bZ); \bZ)\rightarrow H_2(Q; \bZ)$.
Now we have to show that the kernel of this map contains $2 H_2(\Sp(2g, \bZ); \bZ)\cong 2\bZ$.

Note that 
$$\mathsf{ker}\left(p_*\colon H_2(\Sp(2g, \bZ); \bZ)\longrightarrow H_2(Q; \bZ)\right)=\mathsf{ker}\left(p_1\circ\phi\right)\cap  H_2(\Sp(2g, \bZ); \bZ).$$

To conclude, it is thus enough to show that $\mathsf{ker}\left(p_1\circ\phi\right)$ contains $2\bZ$. Thus by Theorem \ref{deligne} it is enough to show that $[\widetilde{\Sp(2g, \bZ)}:\mathsf{ker}\left(p_1\circ\phi\right)]<\infty$.

To this purpose, observe that $$\mathsf{ker}\left(p_1\circ\phi\right)=\phi^{-1}\left(\{\mathrm{id}\}\times K\right)\leq\widetilde{K}=u^{-1}(K)=\phi^{-1}\left(H_2(Q; \bZ)\times K\right).$$
But as $Q$ is finite, we have that $H^2(Q; \bZ)$ is finite (\cite[III, 10.2]{brown} implies that $H^2(Q; \bZ)$ is torsion, and the cohomology of $Q$ is finitely generated). This together with the universal coefficient theorem, as $Q$ is perfect, yields that $H_2(Q; \bZ)$ has no free part (see the diagram below with $A=\bZ$). As the homology of $Q$ is finitely generated as well, the abelian group $H_2(Q; \bZ)$ is finite.

Now note that $$[\phi^{-1}(H_2(Q; \bZ)\times K):\phi^{-1}(\{\mathrm{id}\}\times K)]=[H_2(Q; \bZ)\times K:\{\mathrm{id}\}\times K]=|H_2(Q;\bZ)|<\infty.$$
Thus
$$\begin{array}{ccl}
[\widetilde{\Sp(2g, \bZ)}:\mathsf{ker}\left(p_1\circ\phi\right)]&=&[\widetilde{\Sp(2g, \bZ)}:\widetilde{K}][\widetilde{K}:\mathsf{ker}\left(p_1\circ\phi\right)]\\
	&=&[\widetilde{\Sp(2g, \bZ)}:\widetilde{K}][\phi^{-1}(H_2(Q; \bZ)\times K):\phi^{-1}(\{\mathrm{id}\}\times K)]\\
	&=&[\widetilde{\Sp(2g, \bZ)}:\widetilde{K}][H_2(Q; \bZ)\times K:\{\mathrm{id}\}\times K]<\infty
	\end{array}$$
as both factors in the last line are finite.
This proves Claim 1.

As $\Sp(2g, \bZ)$ and $Q$ are perfect, the universal coefficient theorem for cohomology provides the following commutative diagram:
$$\xymatrix{
\mathsf{Hom}(H_2(Q; \bZ), A)\ar[rr]^-{\mathsf{Hom}(p_*)}\ar@{}[d]|*[@]{\cong}& & \mathsf{Hom}(H_2(\Sp(2g, \bZ); \bZ), A)\ar@{}[d]|*[@]{\cong}\\
H^2(Q; A)\ar[rr]^-{p^*}&& H^2(\Sp(2g, \bZ); A)
}$$
for any principal ideal domain $A$.

{\bfseries Claim 2:} $\mathsf{Im}(p^*)\subset T_2(H^2(\Sp(2g, \bZ); A))$, where $T_2$ denotes the $2$-torsion.

{\bfseries Proof of Claim 2:} As indicated by the commutative diagram, the map $p^*$ is defined as follows:
$$ H^2(Q; A)\cong \mathsf{Hom}(H_2(Q; \bZ), A)\ni\alpha\longmapsto \alpha\circ p_*\in \mathsf{Hom}(H_2(\Sp(2g, \bZ); \bZ), A)\cong H^2(\Sp(2g, \bZ); A).$$
Then let $g\geqslant 4$ and $n\in H_2(\Sp(2g, \bZ); \bZ)\cong\bZ$. If $2\mid n$, Claim $1$ implies $p_*(n)=0$. So $\mathsf{Hom}(p_*)(\alpha)$ is determined by $\mathsf{Hom}(p_*)(\alpha)(1)$, and we have
$$2\mathsf{Hom}(p_*)(\alpha)(1)=\mathsf{Hom}(p_*)(\alpha)(2)=0.$$
%If $g=3$, the same proof holds, as the only difference between $g=3$ and $g\geqslant 4$ is an additional $2$-torsion summand in the second homology.

This proves Claim $2$.

Note that $H^2(\Sp(2g, \bZ); A)\cong\mathsf{Hom}(H_2(\Sp(2g, \bZ); \bZ), A)\cong \mathsf{Hom}(\bZ, A)\cong A$ if $g\geqslant 4$.% and
%$$H^2(\mathsf{Sp}(2g, \bZ), A)=A\oplus T_2(A)$$ if $g=3$.

Now comes the final part of the proof. Let $[\tau_g]_A$ denote the image of $[\tau_g]$ in $H^2(\Sp(2g, \bZ); A)$. Suppose that there exists a class $c\in H^2(Q; A)$ such that $$p^*(c)=[\tau_g]_A.$$ By Claim $2$ we have $2p^*(c)=0$. On the other hand, $[\tau_g]_A$ is the image of $[\tau_g]=4\in \bZ\cong H^2(\Sp(2g, \bZ); \bZ)$ in $A$. So we have $$p^*(c)=4_A\in T_2(A).$$

Hence this class $c$ can provide at most the $2$-valued information $4_A$ on the signature: either it is $0$ in $A$ or not.
\end{proof}

\begin{rk}\label{Z/m}
In particular, setting $A=\bZ/N$, we find the following:
$4_N\in T_2(\bZ/N)$, and
$$T_2(\bZ/N)=
\left\{ \begin{array}{ll}
		\{0\}& \mbox{if }N\mbox{ is odd},\\
		\left\{0, \frac{N}{2}\right\}& \mbox{if }N\mbox{ is even}.
		\end{array}
		\right.$$
Hence no information is obtained in this way for odd $N$. For even $N$, suppose $\frac{N}{2}=4_N$. Then 
\begin{eqnarray}
\frac{N}{2}=4\pmod{N}\phantom{.}\\
N \mid \frac{N}{2}-4\phantom{.}\\
\frac{N}{2}-4=qN \mbox{ for some } q\in \mathbb{Z}\phantom{.}\\
N(1-2q)=8\phantom{.}\\
1-2q\mbox{ is odd and divides }8\phantom{.}\\
1-2q=1\phantom{.}\\
q=0.
\end{eqnarray}
So $N=8$.
\end{rk}
%\begin{rk}
%In particular, for such a class $c$ to exist at all, we must have $T_2(A)\neq \{0\}$.
%\end{rk}
\begin{rk}
If $g=3$, the conclusions of Theorems \ref{cas Z/m} and \ref{cas general} still hold, with the same proof, as the only difference between $g=3$ and $g\geqslant 4$ is an additional $2$-torsion summand in the second homology of the symplectic group with integer coefficients (Lemma \ref{Lemma:co-homology computations}\ref{H_2 Sp Z Z}) as well as a $2$-torsion factor in the universal extension of $\Sp(6,\bZ)$ (Theorem \ref{th:main}(xi)).
\end{rk}



==> paper3-bibgeq2.tex <==
%PAPER3-BIB.TEX (14.11.2018)
%OWNER 

\bibliographystyle{amsplan}
\newcommand{\noopsort}[1]{}
\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
\begin{thebibliography}{10}
\bibitem{barge-ghys}
J.~Barge, E.~Ghys, \emph{Cocycles d'Euler et de Maslov}, Math. Ann. \textbf{294} (1992), no.~2, 235--265.

\bibitem{baaj-skandalis-vaes}
S.~Baaj, G.~Skandalis, and S.~Vaes,
\emph{Measurable Kac Cohomology for Bicrossed Products},
Trans. Amer. Math. Soc. \textbf{357} (November 2004), no.~4, 1497--1524.

\bibitem{bender}
P.~Bender, \emph{Eine Pr\"asentation der symplektischen Gruppe $\Sp(4, \bZ)$ mit $2$ Erzeungenden und $8$ definierenden Relationen},
J. Algebra \textbf{65} (1980), no.~2, 328--331.

\bibitem{Benson:theta}
D.~J.~Benson, \emph{Theta functions and a presentation of
  $2^{1+(2g+1)}\mathsf{Sp}(2g,2)$}, J. Algebra \textbf{527} (2019), 204--240.
 
\bibitem{BensonCampagnoloRanickiRovi:2017a}
\bysame, C. Campagnolo, A. Ranicki, and C. Rovi, \emph{Cohomology of symplectic groups and Meyer's signature theorems}, Algebr. Geom. Topol. \textbf{18} (2018), no.~7, 4069--4091.

\bibitem{beyl}
F.~R.~Beyl, \emph{The Schur multiplicator of $\rm {SL}(2,{\bf Z}/m{\bf Z})$ and the Congruence Subgroup Property}, Math. Z. \textbf{191} (1986), no.~1, 23--42.
    
\bibitem{brown}
	K.~S.~Brown, \emph{Cohomology of Groups},
	Springer (1982).

\bibitem{CampagnoloThesis}
C.~Campagnolo,
\emph{Surface bundles over surfaces: A study through signature and simplicial volume},
10.13097/archive-ouverte/unige:96380, 2016.

\bibitem{ChatterjiMislindeCornulierPittet:2013a}
I.~Chatterji, Y.~de Cornulier, G.~Mislin, and C.~Pittet,
\emph{Bounded characteristic classes and flat bundles},
J. Differential. Geom. \textbf{95} (2013), no.~1, 39--51.

\bibitem{ChatterjiMislinPittetSaloff-Coste}
I.~Chatterji, G.~Mislin, C.~Pittet, and L.~Saloff-Coste,
\emph{A geometric criterion for the boundedness of characteristic classes},
Math. Ann. \textbf{351} (2011), no.~3, 541--569.

\bibitem{chern-hirzebruch-serre}
	S. S. Chern, F. Hirzebruch, J.-P. Serre,
	\emph{On the Index of a Fibered Manifold},
	Proceedings of the American Mathematical Society \textbf{8} (Jun., 1957), no.~3, 587--596.

\bibitem{atlas}
J.~H.~Conway, R.~Turner~Curtis, S.~P.~Norton, R.~A.~Parker, and R.~Arnott Wilson,
\emph{Atlas of Finite Groups. Maximal Subgroups and Ordinary Characters for Simple Groups}, 
Oxford University Press, 1985.

\bibitem{Deligne:1978a}
P.~Deligne, \emph{Extensions centrales non r\'esiduellement finies des groupes
  arithm\'etiques}, C. R. Acad. Sci. Paris, S\'er. A-B \textbf{287}
  (1978), no.~4, A203--A208.

\bibitem{Farb/Margalit:2012a}
B.~Farb and D.~Margalit, \emph{A primer on mapping class groups},
Princeton (2012).

\bibitem{galatius-randal-williams}
S.~Galatius and O.~Randal-Williams, \emph{Abelian quotients of mapping class groups of highly connected manifolds}, Math. Ann. \textbf{365} (2016), no.~1-2, 857--879.

\bibitem{Gilmer/Masbaum:2013a}
P.~Gilmer and G.~Masbaum, \emph{Maslov index, lagrangians, mapping class groups and TQFT}, Forum Math. \textbf{25} (2013), no.~5, 1067--1106.

\bibitem{Griess:1973a}
R.~L.~Griess, \emph{Automorphisms of extra special groups and nonvanishing
  degree $2$ cohomology}, Pacific J. Math. \textbf{48} (1973), no.~2,
  403--422.

\bibitem{Hambleton/Korzeniewski/Ranicki:2007a}
I.~Hambleton, A.~Korzeniewski, and A.~Ranicki, \emph{The signature of a fibre
  bundle is multiplicative mod $4$}, Geom. Topol. \textbf{11} (2007),
  251--314.
  
%\bibitem{Harer:1983a}
%J. L.~Harer, \emph{{The second homology group of the mapping class group of an orientable surface}},
%Inv. Math. \textbf{72} (1983), 221--239. 
  
%\bibitem{Harer:1988a}
%\bysame, {{The cohomology of the moduli space of curves}},
%in Theory of Moduli, Lecture Notes in Mathematics \textbf{1337} (1988),
%138--221. 
 
\bibitem{Hochschild:1965a}
G.~Hochschild, \emph{The Structure of Lie Groups},
Holden-Day (1965).

\bibitem{Hopf:1942a}
H.~Hopf, \emph{Fundamentalgruppe und zweite Bettische Gruppe},
Comment. Math. Helv. \textbf{14} (1942), 257--309.

\bibitem{kirby-melvin}
R.~Kirby and P.~Melvin, \emph{Dedekind sums, $\mu$-invariants and the signature cocycle}, Math. Ann. \textbf{299} (1994), no.~2, 231--267.

\bibitem{korkmaz}
M.~Korkmaz, \emph{Low-dimensional homology groups of mapping class groups: a survey}, Turkish J. Math. \textbf{26} (2002), no.~1, 101--114.
  
\bibitem{Korkmaz/Stipsicz:2003a}
M.~Korkmaz and A.~I.~Stipsicz,
\emph{The second homology groups of mapping class groups of orientable surfaces},
Math. Proc. Cambridge Philos. Soc. \textbf{134} (2003), no.~3, 479--489.
  
\bibitem{Leray:1981a}
J.~Leray, \emph{Lagrangian analysis and quantum mechanics},
MIT Press (1981).

\bibitem{lu}
N.~Lu, \emph{A Simple presentation of the Siegel Modular Groups}, Linear Algebra Appl. \textbf{166} (1992), 185--194.

\bibitem{Mackey:1957a}
G.~W.~Mackey, \emph{Borel structure in groups and their duals},
Trans. Amer. Math. Soc. \textbf{85} (1957), 134--165.

\bibitem{Maslov:1965a}
V.~P.~Maslov, \emph{Th\'eorie des perturbations et m\'ethodes asymptotiques}, Dunod (1972 (transl. of 1965 Russian edition)).

\bibitem{Meyer:1972a}
W.~Meyer, \emph{Die Signatur von lokalen Koeffizientensystemen und Faserb\"undeln.},
Bonn. Math. Schr. No. 53 (1972), viii+59,
\href{http://www.maths.ed.ac.uk/~aar/papers/meyerthesis.pdf}{http://www.maths.ed.ac.uk/~aar/papers/meyerthesis.pdf}


\bibitem{Meyer:1973a}
W.~Meyer, \emph{Die Signatur von Fl\"achenb\"undeln}, Math.\ Ann.
  \textbf{201} (1973), 239--264.

\bibitem{Milnor:1983a}
J.~Milnor, \emph{On the homology of Lie groups made discrete},
Comment. Math. Helv. \textbf{58} (1983), no.~1, 72--85.

\bibitem{moore}
C.~C.~Moore,
\emph{Group Extensions and Cohomology for Locally Compact Groups. III},
Trans. Amer. Math. Soc. \textbf{221} (July 1976), no.~1, 1--33.

\bibitem{Py:2005a}
P.~Py, \emph{Indice de Maslov et Th\'eor\`eme de Novikov--Wall},
Bol.\ Soc.\ Mat.\ Mexicana (3) \textbf{11} (2005), no.~2, 303--331.

\bibitem{Rovi:AGT}
C.~Rovi, \emph{The non-multiplicativity of the signature modulo $8$ of a fibre
  bundle is an Arf--Kervaire invariant}, Algebr. Geom. Topol. \textbf{18} (2018), 1281--1322.

\bibitem{Sah/Wagoner:1977a}
C.-H.~Sah and J. B.~Wagoner,
\emph{Second homology of Lie groups made discrete},
Comm. Algebra \textbf{5} (1977), no.~6, 611--642.

\bibitem{sakasai}
T.~Sakasai, \emph{Lagrangian mapping class groups from a group cohomological point of view}, Algebr. Geom. Topol. \textbf{12} (2012), no.~1, 267--291.

\bibitem{Scharlau:2017a}
W.~Scharlau, \emph{Das Gl\"uck, Mathematiker zu sein. Friedrich Hirzebruch und seine Zeit}, 
Heidelberg: Springer Spektrum (2017).

\bibitem{Schur:1904a}
J.~Schur, \emph{\"Uber die Darstellung der endlichen Gruppen durch gebrochene lineare Substitutionen},
J. reine angew. Math. \textbf{127} (1904), 20--50.

\bibitem{Thurston:1974a}
W.~Thurston, \emph{Foliations and groups of diffeomorphisms},
Bull. Amer. Math. Soc. \textbf{80} (1974), 304--307.

\bibitem{Wall:1969a}
C.~T.~C.~Wall, \emph{Non-additivity of the signature},
Invent. Math, \textbf{7} (1969), 269--274.

\bibitem{Weil:1940a}
A.~Weil, \emph{L'int\'egration dans les groupes topologiques et ses applications}, Hermann, Paris (1940).

\bibitem{wigner}
D.~Wigner,
\emph{Algebraic Cohomology of Topological Groups},
Trans. Amer. Math. Soc. \textbf{178} (April 1973), 83--93.

\end{thebibliography}


\end{document}











%PAPER3-6.TEX (2.1.2018)
%OWNER

\section{The symplectic group $\Sp(2g,\bR)$}\label{se:Sp2gR}

In this section, we examine the homotopy type and cohomology of
$\Sp(2g,\bR)$, and use this to compare the cocycles described in
Section \ref{se:Meyer}.

\begin{theorem}\label{th:max-compact}
Let $G$ be a Lie group with finitely many connected components, and let $K$
be a maximal compact subgroup.\index{maximal compact subgroup} 
Then as a topological space,
$G$ is homeomorphic to a Cartesian product $K \times \bR^d$, where $d$ is the
codimension of $K$ in $G$. In particular, the inclusion of
$K$ in $G$ is a homotopy equivalence.
\end{theorem}
\begin{proof}
See Theorem 3.1 in Chapter XV of Hochschild \cite{Hochschild:1965a}.
\end{proof}

In the case of $\Sp(2g,\bR)$, a connected Lie group of dimension $g(2g+1)$, 
the maximal compact subgroup is
the unitary group\index{unitary group} $\UU(g)$ of dimension $g^2$. Thus as a topological space,
we have $\Sp(2g,\bR) \cong \UU(g) \times \bR^{g(g+1)}$.

\begin{prop}\label{pr:UgSp2gR}
The inclusion $\UU(g) \to \Sp(2g,\bR)$ of topological groups is a homotopy equivalence.
Thus we have $\pi_1(\Sp(2g,\bR)) \cong \bZ$ and 
$$ H^*(B\Sp(2g,\bR);\bZ)\cong \bZ[c_1,\dots,c_g], $$
where $c_i\in H^{2i}(B\Sp(2g,\bR);\bZ)=H^{2i}(B\UU(g);\bZ)$ denotes the $i$-th Chern class.
\end{prop}
\begin{proof}
This follows from Theorem \ref{th:max-compact} and 
well known properties of $\UU(g)$.
\end{proof}


\begin{cor}
The coset space $\Sp(2g,\bR)/\Sp(2g-2,\bR)$ is homeomorphic to
a Cartesian product $S^{2g-1} \times \bR^{2g}$.\qed
\end{cor}


\begin{cor}\label{co:pi1Sp}
The inclusions 
$$ S^1=U(1)\to \Sp(2,\bR) \to \Sp(4,\bR) \to \cdots \to \Sp(2g,\bR) $$
induce isomorphisms on $\pi_1$.\qed
\end{cor}



\begin{cor}\label{co:H_b^2Sp}
The Borel cohomology $H_b^2(\Sp(2g,\bR),\bZ)$ is isomorphic to $\bZ$,
with generator $c_1$. The restriction map 
$$ H_b^2(\Sp(2g,\bR),\bZ)\to H_b^2(\Sp(2g-2,\bR),\bZ) $$ 
is an isomorphism.
\end{cor}
\begin{proof}
This follows from the Serre spectral sequence of a fibration and the fact that $\Sp(2g,\bR)/\Sp(2g-2,\bR)$ is $(2g-2)$-connected for $g\geq 2$.
\end{proof}

\begin{theorem}\label{th:tautau'}
The cohomology class in $H^2_b(\Sp(2g,\bR),\bZ) \cong H^2(B\Sp(2g,\bR);\bZ)\cong \bZ$ defined by the
Meyer cocycle $\tau_g$ and the Maslov cocycle $\tau'_g$ are both equal to $4c_1$.
\end{theorem}
\begin{proof}
Remember from Theorem \ref{th:Borel} that $H_b^2(\Sp(2g, \bR), \bZ)\cong H^2(B\Sp(2g,\bR);\bZ)$,  which is $\bZ$ by Proposition \ref{pr:UgSp2gR}, and that it injects into $H^2(\Sp(2g, \bR)^\delta, \bZ)$.
It follows from Proposition \ref{pr:cocycles-restrict} and Corollaries \ref{co:pi1Sp}, \ref{co:H_b^2Sp}
that it suffices to prove the second statement for the subgroup 
$S^1=U(1)\subseteq \Sp(2,\bR)$.
In this case, the Meyer cocycle is represented by the first diagram
in Example \ref{eg:MeyerS1}, while the Maslov cocycle is represented by the second diagram.
According to Theorem \ref{th:S1cocycle}, these both have covering number $4$.
The standard cocycle on $S^{1\delta}$ is Borel and is the restriction of a cocycle on $\Sp(2,\bR)$ representing $c_1$, 
so this has covering number $1$.
\end{proof}


%PAPER3-7.TEX
%OWNER

\section{The signature of a surface bundle modulo eight}\label{se:recipe}


Let $\Sigma_g \to M \to \Sigma_h$ be a surface bundle, with fibre
the surface $\Sigma_g$  of genus $g \geqslant 1$, and base the surface $\Sigma_h$ of genus $h \geqslant 1$.
We shall use the $\bZ/4$-coefficient monodromy
$$\pi_1(\Sigma_h) \to \mcg{g} \to \Sp(2g,\bZ) \to \Sp(2g,\bZ/4)$$
to provide a recipe for computing the signature
of the $4$-manifold $M$ modulo eight.


We start with some generalities about central group extensions and commutators.



For any abelian group $A$ there is defined a cap product pairing
$$H^2(\Sigma_h;A)\otimes H_2(\Sigma_h) \to H_0(\Sigma_h;A)=A~;~(\sigma,[\Sigma_h]) \mapsto
\langle \sigma,[\Sigma_h] \rangle$$
with $[\Sigma_h] \in H_2(\Sigma_h)$ the fundamental class. In the first instance, we obtain a formula for
$\langle \sigma,[\Sigma_h] \rangle \in A$ in terms of the central extension
$$1 \to A \to H \to \pi_1(\Sigma_h) \to 1$$
classified by $\sigma \in H^2(\Sigma_h;A)=H^2(\pi_1(\Sigma_h);A)$. 
The fundamental group of $\Sigma_h$  is the one relator
group\index{one relator group} given by
\[ \pi_1(\Sigma_h)=\langle a_1,b_1,a_2,b_2,\dots,a_h,b_h\mid r\rangle \]
where $r= [a_1,b_1][a_2,b_2]\dots[a_h,b_h]$ is the single relator.



\begin{lemma}\label{le:fundamental} 
{\rm (i)} The central extension classified by $1 \in H^2(\pi_1(\Sigma_h);\bZ)\cong \bZ$ 
$$1 \to \bZ \to \widetilde{\pi_1(\Sigma_h)} \to \pi_1(\Sigma_h) \to 1$$
is given by
$$\begin{array}{l}
\widetilde{\pi_1(\Sigma_h)}~=~\langle a_1,b_1,\dots,a_h,b_h,r\,\vert\, [a_1,r],\dots,[b_h,r],r=[a_1,b_1]\dots[a_h,b_h]\rangle~,\\[1ex]
\bZ \to \widetilde{\pi_1(\Sigma_h)}~;~1 \mapsto r~.
\end{array}$$
{\rm (ii)} Let $1 \to A \to H \to \pi_1(\Sigma_h) \to 1$ be the central extension
classified by $\sigma \in H^2(\Sigma_h;A)\cong H^2(\pi_1(\Sigma_h);A)\cong A$.
There is defined a morphism of central group extensions
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r] \ar[d] & \widetilde{\pi_1(\Sigma_h)} \ar[r] \ar[d]^-{\chi} & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1 \\
1 \ar[r] & A \ar[r] & H \ar[r] & \pi_1(\Sigma_h) \ar[r] & 1} \]
such that 
$\langle \sigma,[\Sigma_h] \rangle\in A$ is the image of $[\Sigma_h]=1\in H_2(\Sigma_h)\cong \bZ$ under the left hand vertical map, with
$$\langle \sigma,[\Sigma_h] \rangle=\chi([a_1,b_1][a_2,b_2] \dots [a_h,b_h]) \in A \subset H~.$$
{\rm (iii)} For any group $\bar{G}$, abelian group $A$ and cohomology class $c \in H^2(\bar{G};A)$ let
$$1 \to A \to G \to \bar{G} \to 1$$
be the central extension of $\bar{G}$ by $A$ classified by $c$. 
A group morphism $\bar{f}:\pi_1(\Sigma_h) \to \bar{G}$ is determined
by elements $u_1,v_1,\dots,u_h,v_h \in  G$ such that
$[u_1,v_1]\dots [u_h,v_h] \in A$, with $\bar{f}(a_i)=u_i$, $\bar{f}(b_i)=v_i$. The pullback central extension $H$ of $\pi_1(\Sigma_h)$ by $A$
\[ \xymatrix@R=6mm{1 \ar[r] & A \ar[r] \ar@{=}[d] & H \ar[r] \ar[d]^-{f} & \pi_1(\Sigma_h) \ar[r] \ar[d]^-{\bar{f}} & 1 \\
1 \ar[r] & A \ar[r] &  G\ar[r]  & \bar{G} \ar[r] & 1} \]
is classified by
$$\bar{f}^*(c)= [u_1,v_1]\dots [u_h,v_h] \in H^2(\pi_1(\Sigma_h);A)\cong A~.$$
\end{lemma}
\begin{proof} (i) By construction.\\
(ii) We begin with the observation that since $h\geqslant 1$, $\Sigma_h$ is
a $K(\pi_1(\Sigma_h),1)$, so that
$$H_1(\pi_1(\Sigma_h))=H_1(\Sigma_h)=\bZ^{2h}~,~H_2(\pi_1(\Sigma_h))=H_2(\Sigma_h)=\bZ~.$$
In particular,
\[ \Ext^1_{\bZ}(H_1(\pi_1(\Sigma_h)),H_2(\pi_1(\Sigma_h)))=0, \]
and so the Universal Coefficient Sequence shows that
\[ H^2(\pi_1(\Sigma_h),H_2(\pi_1(\Sigma_h))) \to \Hom_\bZ(H_2(\pi_1(\Sigma_h)),H_2(\pi_1(\Sigma_h))) \]
is an isomorphism. In particular, lifting the identity homomorphism gives
a well defined generator of $H^2(\pi_1(\Sigma_h),\bZ)\cong \bZ$,
corresponding to the  central extension  $1 \to \bZ \to \widetilde{\pi_1(\Sigma_h)} \to \pi_1(\Sigma_h) \to 1$ of (i). The recipe of Hopf \cite{Hopf:1942a} for computing $H_2(G)$, which is the
same as the recipe of Schur \cite{Schur:1904a} for the multiplier of $G$, is that if $G$ is a quotient of a free group $F$ by relations $R$ then $H_2(G)=R\cap[F,F]/[F,R]$. If $R\subseteq [F,F]$ there is a canonical central
extension
$$1 \to H_2(G)=R/[R,F] \to \widetilde{G}=F/[R,F] \to G=F/R \to 1$$
classified by $1 \in H^2(G;H_2(G)) \cong  \Hom(H_2(G),H_2(G))$.
In particular, for $G=\pi_1(\Sigma_h)$, $H_2(G)=\bZ$ this gives the extension $\widetilde{\pi_1(\Sigma_h)}$
with the presentation in the statement of (i).\\
\indent Now given an abelian group $A$ and an element $\sigma\in H^2(\pi_1(\Sigma_h),A)$, we can evaluate
$\sigma$ on $[\Sigma_h]$ as follows. Since $\widetilde{\pi_1(\Sigma_h)}$ is universal, we obtain a lifting
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r] \ar[d] & \widetilde{\pi_1(\Sigma_h)} \ar[r] \ar[d] & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1 \\
1 \ar[r] & A \ar[r] & H \ar[r] & \pi_1(\Sigma_h) \ar[r] & 1} \]
with $\bZ \to A;1 \mapsto \langle \sigma,[\Sigma_h] \rangle$.\\
{\rm (iii)} Apply (i) and (ii) with $\sigma=\bar{f}^*(c) \in H^2(\pi_1(\Sigma_h);A)$: consider the commutative diagram
\[ \xymatrix@R=6mm{1 \ar[r] & \bZ \ar[r] \ar[d] & \widetilde{\pi_1(\Sigma_h)} \ar[r] \ar[d]^-{\chi} & \pi_1(\Sigma_h) \ar[r] \ar@{=}[d] & 1 \\
1 \ar[r] & A \ar[r] \ar@{=}[d] & H \ar[r] \ar[d]^-{f} & \pi_1(\Sigma_h) \ar[r] \ar[d]^-{\bar{f}} & 1 \\
1 \ar[r] & A \ar[r] & G\ar[r]  & \bar{G} \ar[r] & 1} \]
and note that
\begin{align*}
\langle \bar{f}^*(c),[\Sigma_h] \rangle
&=\chi([a_1,b_1][a_2,b_2] \dots [a_h,b_h]) \\
&=[u_1,v_1]\dots [u_h,v_h] \in H^2(\pi_1(\Sigma_h);A)\cong A~.
\qedhere
\end{align*}
\end{proof}


Let $N \geqslant 0$; for $N=0$ $\bZ/N$ is the infinite cyclic group, and for $N \geqslant 1$ $\bZ/N$ is the finite cyclic group of order $N$. 

\begin{eg}\label{le:extensionbyzN}
The central extension
$$1 \to \bZ/N \to \widetilde{\pi_1(\Sigma_h)} \to \pi_1(\Sigma_h) \to 1$$
classified by $1 \in H^2(\pi_1(\Sigma_h);\bZ/N)=\bZ/N$ is
$$\begin{array}{l}
\widetilde{\pi_1(\Sigma_h)}~=~\langle a_1,b_1,\dots,a_h,b_h,r\,\vert\, [a_1,r],\dots,[b_h,r],r=[a_1,b_1]\dots[a_h,b_h],r^N\rangle~,\\[1ex]
\bZ/N \to \widetilde{\pi_1(\Sigma_h)}~;~1 \mapsto r~.
\end{array}$$
\hfill\qed
\end{eg}

Meyer \cite{Meyer:1973a} proved that $\sigma(M)=0$ for a surface bundle $\Sigma_g \to M \to \Sigma_h$ with $g \leqslant 2$. 

\begin{lemma} \label{le:symplectic}
Let $g \geqslant 3$.\\
{\rm (i)} The cohomology class
$$[\tau]=4 \in H^2(\Sp(2g,\bZ),\bZ) \cong  \bZ$$
 corresponds to the canonical central extension
\[ 1 \to \bZ \to \widetilde{\Sp(2g,\bZ)} \to \Sp(2g,\bZ) \to 1\]
with cocycle determined by the signatures of the double mapping tori
$$c:\Sp(2g,\bZ) \times \Sp(2g,\bZ) \to \bZ;(\alpha,\beta) \mapsto
\sigma(T(\alpha,\beta))~.$$
{\rm (ii)} For a surface bundle $F=\Sigma_g \to M \to B=\Sigma_h$
$$\sigma(M)=\langle \bar\chi^*([\tau]),[\Sigma_h] \rangle \in 4\bZ$$
with $\bar\chi:\pi_1(\Sigma_h) \to \Sp(2g,\bZ)$ the monodromy. The cohomology class
$\bar\chi^*([\tau]) \in H^2(\pi_1(\Sigma_h),\bZ)$ classifies the extension
$$1 \to \bZ \to \widetilde{\pi_1(\Sigma_h)} \to \pi_1(\Sigma_h) \to 1$$
with cocycle
$$\pi_1(\Sigma_h) \times \pi_1(\Sigma_h) \to \bZ ~;~
(\alpha,\beta) \mapsto \sigma(T(\chi(\alpha),\chi(\beta)))~.$$
For $\bar \chi(a_i)=u_i$, $\bar \chi(b_i)=v_i \in Sp(2g,\bZ)$
this is the pullback of the central extension of $\Sp(2g,\bZ)$ in {\rm (i)}
$$\xymatrix{
1 \ar[r] & \bZ \ar@{=}[d] \ar[r] & \widetilde{\pi_1(\Sigma_h)} \ar[r] \ar[d] & \pi_1(\Sigma_h) \ar[d]^{\displaystyle{\bar\chi}} \ar[r] & 1 \\
1 \ar[r] & \bZ \ar[r] & \widetilde{\Sp(2g,\bZ)} \ar[r]^-{\displaystyle{p}} & \Sp(2g,\bZ)\ar[r] & 1}$$
with 
$$(\sigma(M),1)~=~
(0,[u_1,v_1])(0,[u_2,v_2]) \dots (0,[u_h,v_h]) \in
\widetilde{\Sp(2g,\bZ)}~.$$
{\rm (iii)} The $\bZ/2$-reduction  of $[\tau]/4$
$$[\tau]/4=\begin{cases}
(1,0)\\
1 \\
\end{cases} \in
H^2(\Sp(2g,\bZ),\bZ/2) \cong \begin{cases} 
\bZ/2 \oplus \bZ/2  & g=3 \\
  \bZ/2 & g\geqslant 4 \end{cases}$$
 corresponds to the canonical central extension
\[ 1 \to \bZ/2 \to \widetilde{\widetilde{\Sp(2g,\bZ)}} \to \Sp(2g,\bZ) \to 1\]
such that for a surface bundle $\Sigma_g \to M \to \Sigma_h$
$$\sigma(M)/4=\langle \bar \chi^*([\tau]/4),[\Sigma_h] \rangle \in \bZ/2~.$$
\end{lemma}
\begin{proof} (i)+(ii) Meyer \cite{Meyer:1973a}.\\
(iii) Immediate from (ii) and ?? %Theorem \ref{th:H}.
\end{proof}


%PAPER3-8.TEX (2.1.2018)
%OWNER

\section{What about signatures of surface bundles mod $N$ for $N>8$?}
%$$\includegraphics[page=1,width=18cm]{DeligneConsequence.pdf}$$
%$$\includegraphics[page=2,width=18cm]{DeligneConsequence.pdf}$$
%$$\includegraphics[page=3,width=18cm]{DeligneConsequence.pdf}$$
%$$\includegraphics[page=4,width=18cm]{DeligneConsequence.pdf}$$
%$$\includegraphics[page=5,width=18cm]{DeligneConsequence.pdf}$$


In \cite{BensonCampagnoloRanickiRovi:2017a} we showed the existence of a cohomology class in the second cohomology group of a finite quotient of $\mathrm{Sp}(2g, \bZ)$ that computes the $2$-valued invariant which is the signature of surface bundles over surfaces modulo $8$.

Here we explain in detail why this information on the signature is the best we can hope for if we restrict ourselves to cohomology classes on finite quotients of the symplectic group.

Precisely, we want to show the following:
\begin{theorem}\label{cas Z/m}
Let $g\geq 4$ and $K\leq \mathrm{Sp}(2g, \bZ)$ be a normal subgroup of finite index. %in $\mathrm{Sp}(2g, \bZ)$.
If $c \in H^2(\mathrm{Sp}(2g,\bZ)/K,\bZ/m)$ is a cohomology class such that for the monodromy $\chi:\pi_1(\Sigma_h)\rightarrow\mathrm{Sp}(2g,\bZ)$ of any surface bundle $\Sigma_g\rightarrow M\rightarrow\Sigma_h$ we have $$\sigma(M) = \langle\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/m,$$
%and $\langle\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/m$ is not constant equal to $0$
then $m=2, 4,$ or $8$. If $m=2$ or $4$, the value $\langle\chi^*p^*(c),[\Sigma_h]\rangle \in\bZ/m$ is always $0$. Here $p:\mathrm{Sp}(2g,\bZ)\rightarrow\mathrm{Sp}(2g,\bZ)/K$ denotes the quotient map.
\end{theorem}
This will be a direct consequence of a more general result (see also Remark \ref{Z/m}):
\begin{theorem}\label{cas general}
Let $g\geq 4$ and $K\leq \mathrm{Sp}(2g, \bZ)$ be a normal subgroup of finite index, and $A$ be a commutative ring. If $c \in H^2(\mathrm{Sp}(2g,\bZ)/K, A)$ is a cohomology class such that for the monodromy $\chi:\pi_1(\Sigma_h)\rightarrow\mathrm{Sp}(2g,\bZ)$ of any surface bundle $\Sigma_g\rightarrow M\rightarrow\Sigma_h$ we have $$\sigma(M) = \langle\chi^*p^*(c),[\Sigma_h]\rangle \in A,$$
then $\langle\chi^*p^*(c),[\Sigma_h]\rangle$ is the image of $4\in\bZ$ in $A$ and lies in the $2$-torsion of $A$. Here $p:\mathrm{Sp}(2g,\bZ)\rightarrow\mathrm{Sp}(2g,\bZ)/K$ denotes the quotient map.%From the second cohomology of any finite quotient of $\mathrm{Sp}(2g, \bZ)$ with coefficients in any principal ideal domain $A$ one cannot recover more information on the signature of a surface bundle over a surface than a $2$-valued homomorphic image.
\end{theorem}
Morally, this theorem says that any cohomology class on a finite quotient of the symplectic group yields at most a $2$-valued information on the signature of a surface bundle over a surface (as it lies in the $2$-torsion of the arbitrary coefficient ring $A$).

The above results rely on the non-residual finiteness of $\widetilde{\mathrm{Sp}(2g, \bZ)}$  proved by Deligne. We recall the setup.

Let $\widetilde{\mathrm{Sp}(2g, \bZ)}$ denote the central extension obtained by pulling back the universal cover of $\mathrm{Sp}(2g, \mathbb{R})$ to $\mathrm{Sp}(2g, \bZ)$:
$$\xymatrix{
1\ar[r]&\bZ\ar[r]\ar@{=}[d]&\widetilde{\mathrm{Sp}(2g, \bZ)}\ar[r]_u\ar[d]&\mathrm{Sp}(2g, \bZ)\ar[r]\ar[d]&1\\
1\ar[r]&\bZ\ar[r]&\widetilde{\mathrm{Sp}(2g, \mathbb{R})}\ar[r]&\mathrm{Sp}(2g, \mathbb{R})\ar[r]&1
}$$
For $g\geq 4$, the group $\widetilde{\mathrm{Sp}(2g, \bZ)}$ is the universal central extension of the perfect group $\mathrm{Sp}(2g, \bZ)$.

Let $[\tau]\in H^2(\mathrm{Sp}(2g, \bZ), \bZ)$ denote the class of the Meyer signature cocycle. Recall that $[\tau]=4\in\bZ\cong H^2(\mathrm{Sp}(2g, \bZ), \bZ)$ for $g\geq 3$.
\begin{theorem}[Deligne]\label{deligne}
For $g\geq 2$, the group $\widetilde{\mathrm{Sp}(2g, \bZ)}$ is not residually finite: every subgroup of finite index contains the subgroup $2\bZ$.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{cas general}]
Let $Q=\mathrm{Sp}(2g,\bZ)/K$ be a finite quotient of $\mathrm{Sp}(2g, \bZ)$. Denote by $p:\mathrm{Sp}(2g,\bZ)\rightarrow Q$ the projection map. We have a natural isomorphism 
$$\begin{array}{ccc}
\widetilde{\mathrm{Sp}(2g, \bZ)}/\widetilde{K}&\longrightarrow &\mathrm{Sp}(2g, \bZ)/K\\
\widetilde{g}\widetilde{K}&\longmapsto &u(\tilde{g})K,
\end{array}$$
where $\widetilde{K}=u^{-1}(K)$ denotes the preimage of $K$ in $\widetilde{\mathrm{Sp}(2g, \bZ)}$. So $[\widetilde{\mathrm{Sp}(2g, \bZ)}:\widetilde{K}]<\infty$. By Theorem \ref{deligne}, the subgroup $\widetilde{K}$ then contains $2\bZ$.

Note that as $\widetilde{\mathrm{Sp}(2g, \bZ)}$ is the universal central extension of $\mathrm{Sp}(2g, \bZ)$ for $g\geq 4$, the central subgroup of the extension is isomorphic to the second homology group:
$$\bZ\cong H_2(\mathrm{Sp}(2g, \bZ), \bZ),\, \forall g\geq 4.$$
%For $g=3$, we have
%$$\bZ\oplus\bZ/2\bZ\cong H_2(\mathrm{Sp}(2g, \bZ), \bZ).$$

{\bfseries Claim 1:} The map induced by $p$ in homology annihilates the subgroup $2\bZ$:
$$2\bZ\leq \mathrm{Ker}(p_*: H_2(\mathrm{Sp}(2g, \bZ), \bZ)\longrightarrow H_2(Q, \bZ)).$$

{\bfseries Proof of Claim 1:} As a quotient of the perfect group $\mathrm{Sp}(2g, \bZ)$, the group $Q$ is perfect. Hence it possesses a universal central extension $\widetilde{Q}$ satisfying:
$$\xymatrix{
1\ar[r]&H_2(Q, \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1
}$$
Denote by $E$ the pullback of $\widetilde{Q}$ and $\mathrm{Sp}(2g, \bZ)$ fitting in the following comutative diagram:
$$\xymatrix{
1\ar[r]&H_2(Q, \bZ)\times\{id\}\ar[r]\ar[d]_{p_1}& E\ar[d]_{p_1}\ar[r]_-{p_2}& \mathrm{Sp}(2g, \bZ)\ar[r]\ar[d]_p&1\\
1\ar[r]&H_2(Q, \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1
}$$
The maps $p_1$ and $p_2$ denote the projections to the first and the second factor respectively, and $$E=\left\{(\tilde{q}, g)\in\widetilde{Q}\times\mathrm{Sp}(2g, \bZ)\,\vline\, \pi(\tilde{q})=p(g)\right\}.$$
They are both surjective, as $\pi$ and $p$ are. Moreover one checks directly that $E$ is a central extension of $\mathrm{Sp}(2g, \bZ)$. Consequently by the properties of the universal central extension, there exists a unique map $\phi: \widetilde{\mathrm{Sp}(2g, \bZ)}\rightarrow E$ such that $p_2\circ\phi=u$. We now have the commutative diagram
$$\xymatrix{
1\ar[r]&H_2(\mathrm{Sp}(2g, \bZ), \bZ)\ar[r]\ar[d]_{\phi}& \widetilde{\mathrm{Sp}(2g, \bZ)}\ar[d]_{\phi}\ar[dr]^-{u}&&\\
1\ar[r]&H_2(Q, \bZ)\times\{id\}\ar[r]\ar[d]_{p_1}& E\ar[d]_{p_1}\ar[r]_-{p_2}& \mathrm{Sp}(2g, \bZ)\ar[r]\ar[d]_p&1\\
1\ar[r]&H_2(Q, \bZ)\ar[r]&\widetilde{Q}\ar[r]_\pi&Q\ar[r]&1
}$$
By functoriality (and general knowledge on the second homology of perfect groups) the leftmost composition $p_1\circ\phi$ is precisely the induced map in homology $p_*: H_2(\mathrm{Sp}(2g, \bZ), \bZ)\longrightarrow H_2(Q, \bZ)$.
Now we have to show that the kernel of this map contains $2 H_2(\mathrm{Sp}(2g, \bZ), \bZ)\cong 2\bZ$.

Note that 
$$\mathrm{Ker}(p_*: H_2(\mathrm{Sp}(2g, \bZ), \bZ)\longrightarrow H_2(Q, \bZ))=\mathrm{Ker}(p_1\circ\phi)\cap  H_2(\mathrm{Sp}(2g, \bZ), \bZ).$$

To conclude, it is thus enough to show that $\mathrm{Ker}(p_1\circ\phi)$ contains $2\bZ$. Thus by Theorem \ref{deligne} it is enough to show that $[\widetilde{\mathrm{Sp}(2g, \bZ)}:\mathrm{Ker}(p_1\circ\phi)]<\infty$.

To this purpose, observe that $$\mathrm{Ker}(p_1\circ\phi)=\phi^{-1}(\{\mathrm{id}\}\times K)\leq\widetilde{K}=u^{-1}(K)=\phi^{-1}(H_2(Q, \bZ)\times K).$$
But as $Q$ is finite, we have that $H^2(Q, \bZ)$ is finite (\cite[III, 10.2]{brown} implies that $H^2(Q, \bZ)$ is torsion, and the cohomology of $Q$ is finitely generated). This together with the universal coefficient theorem, as $Q$ is perfect, yields that $H_2(Q, \bZ)$ has no free part (see the diagram below with $A=\bZ$). As the homology of $Q$ is finitely generated as well, the abelian group $H_2(Q, \bZ)$ is finite.

Now note that $$[\phi^{-1}(H_2(Q, \bZ)\times K):\phi^{-1}(\{\mathrm{id}\}\times K)]=[H_2(Q, \bZ)\times K:\{\mathrm{id}\}\times K]=|H_2(Q,\bZ)|<\infty.$$
Thus
$$\begin{array}{ccl}
[\widetilde{\mathrm{Sp}(2g, \bZ)}:\mathrm{Ker}(p_1\circ\phi)]&=&[\widetilde{\mathrm{Sp}(2g, \bZ)}:\widetilde{K}][\widetilde{K}:\mathrm{Ker}(p_1\circ\phi)]\\
	&=&[\widetilde{\mathrm{Sp}(2g, \bZ)}:\widetilde{K}][\phi^{-1}(H_2(Q, \bZ)\times K):\phi^{-1}(\{\mathrm{id}\}\times K)]\\
	&=&[\widetilde{\mathrm{Sp}(2g, \bZ)}:\widetilde{K}][H_2(Q, \bZ)\times K:\{\mathrm{id}\}\times K]<\infty
	\end{array}$$
as both factors in the last line are finite.
This proves Claim 1.

As $\mathrm{Sp}(2g, \bZ)$ and $Q$ are perfect, the universal coefficient theorem for cohomology provides the following commutative diagram:
$$\xymatrix{
\mathrm{Hom}(H_2(Q, \bZ), A)\ar[r]_-{\mathrm{Hom}(p_*)}\ar@{}[d]|*[@]{\cong}& \mathrm{Hom}(H_2(\mathrm{Sp}(2g, \bZ), \bZ), A)\ar@{}[d]|*[@]{\cong}\\
H^2(Q, A)\ar[r]^{p^*}& H^2(\mathrm{Sp}(2g, \bZ), A)
}$$
for any principal ideal domain $A$.

{\bfseries Claim 2:} $\mathrm{Im}(p^*)\subset T_2(H^2(\mathrm{Sp}(2g, \bZ), A))$, where $T_2$ denotes the $2$-torsion.

{\bfseries Proof of Claim 2:} As indicated by the commutative diagram, the map $p^*$ is defined as follows:
$$ H^2(Q, A)\cong \mathrm{Hom}(H_2(Q, \bZ), A)\ni\alpha\longmapsto \alpha\circ p_*\in \mathrm{Hom}(H_2(\mathrm{Sp}(2g, \bZ), \bZ), A)\cong H^2(\mathrm{Sp}(2g, \bZ), A).$$
Then let $g\geq 4$ and $n\in H_2(\mathrm{Sp}(2g, \bZ), \bZ)\cong\bZ$. If $2\mid n$, Claim $1$ implies $p_*(n)=0$. So $\mathrm{Hom}(p_*)(\alpha)$ is determined by $\mathrm{Hom}(p_*)(\alpha)(1)$, and we have
$$2\mathrm{Hom}(p_*)(\alpha)(1)=\mathrm{Hom}(p_*)(\alpha)(2)=0.$$
%If $g=3$, the same proof holds, as the only difference between $g=3$ and $g\geq 4$ is an additional $2$-torsion summand in the second homology.

This proves Claim $2$.

Note that $H^2(\mathrm{Sp}(2g, \bZ), A)\cong\mathrm{Hom}(H_2(\mathrm{Sp}(2g, \bZ), \bZ), A)\cong \mathrm{Hom}(\bZ, A)\cong A$ if $g\geq 4$.% and
%$$H^2(\mathrm{Sp}(2g, \bZ), A)=A\oplus T_2(A)$$ if $g=3$.

Now comes the final part of the proof. Let $[\tau]_A$ denote the image of $[\tau]$ in $H^2(\mathrm{Sp}(2g, \bZ), A)$. Suppose that there exists a class $c\in H^2(Q, A)$ such that $$p^*(c)=[\tau]_A.$$ By Claim $2$ we have $2p^*(c)=0$. On the other hand, $[\tau]_A$ is the image of $[\tau]=4\in \bZ\cong H^2(\mathrm{Sp}(2g, \bZ), \bZ)$ in $A$. So we have $$p^*(c)=4_A\in T_2(A).$$

Hence this class $c$ can provide at most the $2$-valued information $4_A$ on the signature: either it is $0$ in $A$ or not.
\end{proof}

\begin{rk}\label{Z/m}
In particular, setting $A=\bZ/m$, we find the following:
$4_m\in T_2(\bZ/m)$, and
$$T_2(\bZ/m)=
\left\{ \begin{array}{ll}
		\{0\}& \mbox{if }m\mbox{ is odd},\\
		\{0, \frac{m}{2}\}& \mbox{if }m\mbox{ is even}.
		\end{array}
		\right.$$
Hence no information is obtained in this way for odd $m$. For even $m$, suppose $\frac{m}{2}=4_m$. Then 
\begin{eqnarray}
\frac{m}{2}=4\pmod{m}\\
m \mid \frac{m}{2}-4\\
\frac{m}{2}-4=qm \mbox{ for some } q\in \mathbb{N}\\
m(1-2q)=8\\
1-2q>0\\
q=0
\end{eqnarray}
So $m=8$.
\end{rk}
%\begin{rk}
%In particular, for such a class $c$ to exist at all, we must have $T_2(A)\neq \{0\}$.
%\end{rk}
\begin{rk}
If $g=3$, the conclusions of Theorems \ref{cas Z/m} and \ref{cas general} still hold, as the only difference between $g=3$ and $g\geq 4$ is an additional $2$-torsion summand in the second homology of the symplectic group with integer coefficients \cite[Tables]{BensonCampagnoloRanickiRovi:2017a}.
\end{rk}





\end{document}

\section{The Lie algebra of the symplectic group}\label{se:symp}

Let $R$ be a commutative ring. For any f.g. free $R$-module $V$ 
define the duality involution
$$T~:~\Hom_R(V,V^*) \to \Hom_R(V,V^*)~;~ \fb \mapsto \fb^*:x \mapsto (y \mapsto
\fb^*(y,x)=\fb(x,y))~.$$
The abelian group of symmetric forms $(V,\fb:V \times V \to R)$ is the $\bZ/2$-cohomology group
$$\begin{array}{ll}
\Symm(V)&=~H^0(\bZ/2;\Hom_R(V,V^*))\\[1ex]
&=~\Ker(1-T:\Hom_R(V,V^*) \to \Hom_R(V,V^*))~.
\end{array}$$
The abelian group of quadratic forms 
$(V,\fb:V \times V \to R,\fq:V \to R)$ is the $\bZ/2$-homology group
$$\begin{array}{ll}
\Quad(V)&=~H_0(\bZ/2;\Hom_R(V,V^*))\\[1ex]
&=~\Coker(1-T:\Hom_R(V,V^*) \to \Hom_R(V,V^*))~.
\end{array}$$
Note there is an isomorphism of $\bZ[\bZ/2]$-modules
$$V^* \otimes_RV^* \to\Hom_R(V,V^*) ~;~f \otimes g \mapsto (x \mapsto (y \mapsto f(x)g(y)))~.$$
with
$$T~:~ V^* \otimes_R V^* \to V^* \otimes_R V^*~;~ f \otimes g \mapsto g \otimes f~.$$

\begin{defn}
The \emph{divided square}\index{divided square, $D^2(V)$} and
\emph{symmetric square} \index{symmetric square, $S^2(V)$} of 
a  f.g. free $R$-module $V$ are the abelian groups
$$\begin{array}{l}
D^2(V) = \Symm(V^*)= H^0(\bZ/2;V \otimes_R V)=
\Ker(1-T:V \otimes_R V \to V \otimes_R V)~,\\[1ex]
S^2(V) =\Quad(V^*)= H_0(\bZ/2;V \otimes_R V)=
\Coker(1-T:V \otimes_R V \to V \otimes_R V)~.
\end{array}$$
\hfill\qed
\end{defn}

As in  \S\ref{se:forms} identify $V \otimes_RV=\Hom_R(V^*,V)$, so that an element of $D^2(V)$ is a symmetric
form $(\fb:V^* \times V^* \to R) \in \Symm(V^*)$, and an element of $S^2(V)$ is a quadratic
form $(\fb:V^* \times V^* \to R,\fq:V^* \to R) \in \Quad(V^*)$.

The Lie algebra $\fsp(2g,R)$ consists of the $2g \times 2g$ matrices $Y$ with entries in $R$, and satisfying
$$ JY+Y^tJ=0 $$
(the vanishing of the linear term in $(I+Y)^tJ(I+Y)$). Thus
$$Y= \begin{pmatrix} A & B \\ C & D \end{pmatrix}:V=L \oplus L^* \to V=L \oplus L^*$$ 
with 
$$JY+Y^*J=\begin{pmatrix} C-C^t & A^t+D \\ -A-D^t & -B+B^t \end{pmatrix}=\begin{pmatrix} 0 & 0 \\ 0 & 0 \end{pmatrix}$$
so that  $B=B^t \in D^2(L^*)$, $C=C^t \in D^2(L)$ 
define symmetric forms $(L,B)$, $(L^*,C)$ and $D=-A^t$.
Putting this together, we see that
$$ (B,C,A) \in D^2(V)=D^2(L) \oplus D^2(L^*) \oplus (L \otimes_R L^*) $$
can be regarded as a symmetric form on $V^*=L^*\oplus L$
$$\fb=\begin{pmatrix}
B & A\\
A^t & C \end{pmatrix}~:~ V^* \times V^* \to R~;~((f,x),(f',x')) \mapsto A(x,f')+A(x',f)+B(f,f')+C(x,x')~.$$
The function
$$\fsp(2g,R) \to D^2(V)=\Symm(V^*)~;~Y \mapsto \begin{pmatrix}
B & A\\
A^t & C \end{pmatrix}$$
is a bijection. More abstractly, if $v\in V$ then the symmetric tensor $v\otimes v$ is identified with the endomorphism sending $x$ to $\langle v,x\rangle v$. Polarising, this identifies
$v\otimes v' + v' \otimes v$ with the endomorphism of $V$ sending
$x$ to $\langle v,x\rangle v' + \langle v',x\rangle v$.
We have therefore proved the following.

\begin{theorem}\label{th:sp2gR-D2V}
For any commutative ring $R$ and f.g. free $R$-module $V$
we have isomorphisms
$$ \fsp(2g,R)\cong D^2(V) \cong R^{g(2g+1)}. $$
The first isomorphism is an isomorphism of $\Sp(2g,R)$-modules, while the
second is an isomorphism of $R$-modules.
\end{theorem}


